Landmarks and Regions: A Robust Approach to Data Extraction

We propose a new approach to extracting data items or field values from semi-structured documents. Examples of such problems include extracting passenger name, departure time and departure airport from a travel itinerary, or extracting price of an item from a purchase receipt. Traditional approaches to data extraction use machine learning or program synthesis to process the whole document to extract the desired fields. Such approaches are not robust to format changes in the document, and the extraction process typically fails even if changes are made to parts of the document that are unrelated to the desired fields of interest. We propose a new approach to data extraction based on the concepts of landmarks and regions. Humans routinely use landmarks in manual processing of documents to zoom in and focus their attention on small regions of interest in the document. Inspired by this human intuition, we use the notion of landmarks in program synthesis to automatically synthesize extraction programs that first extract a small region of interest, and then automatically extract the desired value from the region in a subsequent step. We have implemented our landmark-based extraction approach in a tool LRSyn, and show extensive evaluation on documents in HTML as well as scanned images of invoices and receipts. Our results show that our approach is robust to various types of format changes that routinely happen in real-world settings.

==> old_stuff.tex <==

\begin{comment}
\State $\RegionSpec \gets$ \par
      \hspace*{1.5em}$\{ (\doc, \landmark_i) \mapsto
          \encr(\landmark_i, \annotation(\doc)) \mid \doc \in \cluster_i
      \}$
  \label{line:region-spec}
%
\State $\bpvalue_i \gets
    \mathsf{Average}(\{ \blueprint(\RegionSpec(\doc))) \mid \doc \in \cluster \})$
%
\State $\RProg_i \gets \mathsf{Synthesize}(\RegionSpec, \LL_{rg})$
  \label{line:region-synth}
%
\State $\ExtractionSpec \gets$ \par
      \hspace*{1.5em}$\{ \RegionSpec(\doc, \landmark_i) \mapsto
        \aggregate(\annotation(\doc)) \mid \doc \in \cluster_i
      \}$
%
\State $\EProg_i \gets \mathsf{Synthesize}(\ExtractionSpec, \LL_{ex})$
%
\end{comment}

\begin{comment}
\begin{algorithm}
\small
\caption{Joint clustering and learning landmarks}
\label{algo:joint-clustering-landmarks}
\begin{algorithmic}[2]
\State \JointClusterAndLandmark( $\dtr, \annotation,f_T$ )
\Require Training data $D_{tr}$
\Require Annotation $\annotation(d)$ for each document $d \in D_{tr}$
\Require Field $f_T$

\State (* Initial clustering using whole document blueprints *)
\State for each  document $d \in D$  
\State  \quad $F[d] :=  \blueprint(d, d)$ 
\State  $[C] =  Cluster(D, \lambda d_1, d_2.\fpd(F[d_1], F[d_2]))$ 
\State
\State (* Calculate landmark candidates for each cluster *)
\State (* Calculate landmark-blueprint pairs for each document*)
\State for each cluster $C_i \in [C] :$ 
\State \quad $M_i$=  \LearnLandmarkCandidates($C_i, f_T$)
\State \quad for each document $d \in C_i$
\State \quad \quad $LF[d] := \{ \}$
\State \quad \quad for each landmark $m \in M_i$:
\State \quad \quad \quad $(R,a) := \annotation(d)$ 
\State \quad \quad \quad $R := \encr(R \cup \locate(m,d), d))$
\State \quad \quad  \quad $LF[d] := LF[d] \cup {(m, \blueprint(R, d))}$
\State
\State (*Calculate distances between all pairs of documents *)
\State (* using blueprints on regions when landmarks match *)
\State for all pairs of documents $d_1, d_2 \in D$
\State \quad $dist[d1, d2] := INFINITY$
\State \quad for all $(m_1, f_1) \in LF[d1], (m_2, f_2) \in LF[d2])$
\State \quad \quad if $(m_1 = m_2)$ then
\State \quad \quad \quad  $dist[d1, d2] = min(dist[d_1, d_2], \fpd(f_1, f_2))$
\State
\State (*merge clusters when distance between clusters is below threshold*)
\State Repeat until no change in $[C]$
\State \quad for each pair of clusters $C_1, C_2 \in [C]$
\State \quad dist = average over all $d_1 \in C_1, d_2 \in C_2: dist[d_1, d_2]$
\State \quad if (dist < threshold)
\State \quad \quad (* merge $C_1$ and $C_2$ *)
\State \quad \quad $[C] := [C] \setminus \{C_1, C_2\} \cup (C_1 \cup C_2)$
\State \Return $[C]$
\end{algorithmic}
\end{algorithm}
\end{comment}

Lines 2-6 do an initial
clustering, where each document is given a blueprint based on the whole
document structure (line 4). The clustering subroutine in line 5 takes a
distance function as the second argument, which when given two documents,
computes the distance between the two documents using distance between their
blueprints.

In Lines 9-16, for each cluster $C$, We learn candidate landmarks (line 10). The
subroutine \LearnLandmarkCandidates\ is described in detail later. 
Then, for each document in $d \in C$, and for each candidate landmark $m$, we
calculate the enclosing region containing the landmark as well as the field
values (as given by annotation of $d$), and compute the blueprint of the
region. Then, we store the set of such landmark-blueprint pairs in $LF[d]$
(line 16).

In lines 20-24, we define a distance metric between all pairs of documents $d_1$
and $d_2$, as minimum distance between blueprints of matching landmark
candidates in $LF[d_1]$ and $LF[d_2]$.

Finally, in lines 27-32, we iteratively merge clusters that are close to each
other as measure by the distance metric defined above. Each cluster $C_i$ is a
triple which consists of a list of documents in it, landmark value and the
corresponding region blueprint.

\begin{algorithm}
\small
\caption{Learn landmark candidates}
\label{algo:landmarks}
\begin{algorithmic}[1]
\State \LearnLandmarkCandidates $(C, f_T)$
\Require Cluster $C$, with annotations
\Require Field $f_T$
\State $cand \gets \mathsf{GetCandidates}(C, f_T)$
\State $S \gets \langle\rangle$
\State for each $m  \in cand$
\State \quad $score \gets 0$
\For {$d \in C$}
\State \quad \quad $score \gets score + \mathsf{ScoringFunction}(d, f(d), l)$
\State \quad $S \gets S + \langle l, score \rangle$
\EndFor
\State $cand \gets$ top $k$ candidate landmarks from $S$ sorted by score
\Return $cand$
\end{algorithmic}
\end{algorithm}


Algorithm~\ref{algo:landmarks}~describes
the subroutine \LearnLandmarkCandidates, which is used in Line 9 of Algorithm~\ref{algo:joint-clustering-landmarks}.
Recall that a landmark can be characterized by following properties: (1)the landmark value is present in all the training documents $C$, and (2) the landmark value is near the field values in all the documents.
 The inputs for this algorithm are the annotated training documents from one cluster $C$ and the field $f_T$. The first step of the algorithm generates candidates from the given input documents. The second step iterates over all these candidates and computes its scores for each document using a scoring function. The scoring function itself is domain-specific and we provide more details in the next sub-section. The function return the top $k$ landmarks sorted by their scores (descending). In our experiments, we use $k = 3$.

 Algorithm~\ref{algo:lrsyn-execute}~outlines the steps during execution of the synthesized extraction program with a new document $d$, and landmark value $m$. The execution uses $\locate(d,m)$ to find the location $\ell^m_{d}$ of landmark $m$ in $d$, and constructs a region $R_d$ using as $P_{rg}(\ell^m_{d})$. 
 In line 4, we check if the blueprint of the extraction region $R_d$ is sufficiently close to the blueprint $f$ we saw in the training data used to synthesize the extraction program. If the distance between the two blueprints is above a threshold value, we fail the execution, since we do not have confidence in the correctness of extraction in such a case. If the blueprint of $R_d$ is sufficiently close to $f$, then we execute $P_{ex}$ with the region $R_d$ as argument to extract the desired field value.

\begin{algorithm}
\small
\caption{Execute Extraction Program}
\label{algo:lrsyn-execute}
\begin{algorithmic}[1]
\State \ExecuteExtraction ($d, m, P_{rg}, f, P_{ex}$)
\Require Test document $d$ 
\Require Landmark value $m$
\Require Region Program $P_{rg}$
\Require Region Blueprint $f$
\Require Extraction Program $P_{ex}$
\State $\ell^m \gets \locate(d, m)$
\State $\mathsf{R_d} \gets P_{rg}(d, m)$
\State if $\fpd(\blueprint(R_d, d), f)$ > threshold  
\State \quad return ("failure, cannot process d")
\State $v \gets P_{ex}(R_d)$ \Comment{Extract value from the region}
\State $\Return~v$
\end{algorithmic}
\end{algorithm}


\begin{comment}
\begin{definition}[\textbf{Region of interest}]
Given a tuple ($D$, $L$, $f$) consisting of a document $D$, a landmark $L$ and field $f$, a region of interest $\regionofinterest$: $D \to D_{sub}$ is a function that maps a document to a sub-document such that it is the smallest region encompassing $L$ and $f$.
\end{definition}
\noindent A given document can consists of multiple region of interests $\regionofinterest_1 \ldots \regionofinterest_k$ and multiple occurrences of landmark values. The notion of \textbf{smallest} region is application dependent. For instance, in HTML setting, the smallest region can be a \textit{table row} or a \textit{div} element. We refer to the process of computing this smallest region given a landmark and a field value as \emph{region-growing}.
\end{comment}

\begin{comment}


\begin{example}
In the HTML extraction scenario as shown in Figure~\ref{}, the orange regions denote the \textbf{landmark(s)} $\landmark$ strings. For instance, for extracting the \emph{names of passengers}, a good hierarchical landmark would be \textit{NAME(S) OF PEOPLE TRAVELLING} as underlined by orange followed by the nearest \textit{Name} string. In this case, only \textit{Name} string would not suffice as there is one more occurrence of the same down below (show this in the image). Likewise, for extracting the flight departure times, \textit{Depart} is a good landmark. A landmark is good if it's "near" to the output, disambiguating and also present in all the documents of the said format.

The green boxes indicate the $\regionofinterest$ regions. These regions encompass the landmark strings and the output regions.
\end{example}

\begin{example}
In the Forms extraction scenario as shown in Figure~\ref{}, the orange regions denote the \textbf{landmark(s)} $\landmark$ strings. For instance, for extracting the \emph{Invoice address}, a good landmark would be \textit{INVOICE TO} as shown in the orange. Likewise, for extracting the sales invoice number, \textit{SALES INVOICE} is a good landmark. The green boxes indicate the $\regionofinterest$ regions. These regions encompass the landmark strings and the output regions.
\end{example}


\paragraph{The Hierarchical Extraction Problem}
We now define the Hierarchical extraction problem.
As input, an extraction framework is provided:
\begin{inparaenum}[(a)]
\item inputs $D$ from a data-set,
\item an initial set of \emph{training inputs} $D_{tr} \subseteq D$, which are annotated by human annotators,
\end{inparaenum}

For a field $f$ of type $\type$, the extraction framework is expected to output 
a partial function $f^* : D \not\to \type$. The extraction framework also outputs the clustering and region-growing criteria for $D$ and landmarks $L$ associated with each cluster and field.
%
The quality of the output $f^*$ is measured using the following metrics:
\begin{compactitem}
%\item \emph{Annotation Burden.} This metric measures the number of calls to the
%  annotation oracle $\mathsf{AOracle}$.
\item \emph{Precision $p$.} This is the standard measure of false positives used in
  information retrieval, and is defined as:
% %\textcolor{blue}{
  \[
  p = \frac
    {\mathbf{card}\left(\{ i \in D  \mid f(i) = f^*(i) \wedge f^*(i) \neq \bot \}\right) }
    {\mathbf{card}\left(\{ i \in D \mid f^*(i) \neq \bot \}\right)}.
  \]
%  %}
\item \emph{Recall $r$.} This is the standard measure of false negatives used in
  information retrieval, and is defined as:
%  \textcolor{blue}{
  \[
  r = \frac
    {\mathbf{card}\left(\{ i \in D  \mid f(i) = f^*(i) \wedge f^*(i) \neq \bot \}\right) }
    {\mathbf{card}\left(\{ i \in D \mid f(i) \neq \bot \}\right)}.
  \]
%  }
  \item \emph{F1 score.} This measure combines precision and recall into a single number, and
  is computed as $2 p r / (p + r)$.
\end{compactitem}
\end{comment}

\begin{comment}
\paragraph{Examples and Extraction}
%
An \emph{extraction example} $\ex$ is a pair $\idoc \mapsto
\oregion_0\ldots\oregion_n$ that associates an \emph{input document} $\doc$
with a sequence of \emph{output regions} $\oregion_0\ldots\oregion_n$.
%
The \emph{extraction task} associated with a set of (training) examples
$\Examples = \{ \ex_0, \ldots, \ex_n \}$ is to learn an
\emph{extractor} $\Extractor$ that maps each document $\doc \in \docs$ to a
sequence $\region_0\ldots\region_m \in \Regions(\doc)$.
%
A learner $\learner$ is a procedure to solve the extraction task.
%
The extractor $\Extractor$ is \emph{sound} for $\Examples$ if for each
example $\idoc \mapsto \oregion_0\ldots\oregion_n$, we have that
$\Extractor(\idoc) = \oregion_0\ldots\oregion_n$.
\end{comment}
%%comment

\begin{comment}
Let $\docs$ be the set of all documents and we represent a single document by $\doc$. The exact type of document depends on the application domain, e.g., in a web extraction setting a document will be an HTML DOM tree~\ref{}. Similarly, in a forms extraction setting, a document will be a structured forms image~\ref{}. Within a document set (HTML, Forms), the documents can be comprised of varied formats. For instance, all flight emails of American airlines. We denote each such grouping of documents as $\doc_C_i$. Each group or cluster of documents can in turn contain varied formats.

We assume that a document is composed of potentially overlapping
\emph{regions} (denoted by $\region$).
%
Regions may be logical fragments of a document that do not necessarily
correspond to the structure of the underlying document type.
%
For example, in a HTML DOM tree, each node (element) is a region on its own.
%
Additionally, we also consider certain collections of DOM nodes to be a
logical region: a column of a HTML table is a region though there is no
single structural component (DOM node) that corresponds to a HTML table
column.
%
We denote the set of all regions in a document $\doc$ by $\Regions(\doc)$.
\end{comment}

\begin{comment}
We assume that the application domain is equipped with a \emph{containment
relation} on the regions of a document.
%
Again, the definition of the containment relation is specific to the
application domain.
%
For example, in the HTML domain, we say that $\region_1 \containedin
\region_2$ if every DOM node in $\region_1$ is a descendant of some DOM node
in $\region_2$.
%
For regions $\region_1, \region_2 \in \Regions(\doc)$, we write $\region_1
\containedin \region_2$ to denote that $\region_1$ is contained in region
$\region_2$.
%
\end{comment}

\begin{comment}
\begin{definition}[\textbf{Fields of interest}]
Given a document $\doc$, we define a Field of interest $\field$ as regions we want to extract from it. 
\end{definition}
\noindent A given document can consists of multiple fields of interest $\oregion_0\ldots\oregion_n$. For instance, in Figure~{1}, all the highlighted parts in green form the potential fields of interest.
\end{comment}


\begin{comment}
\begin{figure}[H]
  \begin{tikzpicture}[
    every node/.style={draw,thick,rounded corners=1ex}
  ]
    \node (pic) {\includegraphics[scale=0.3]{images/t.delta.png}} ;

    \node[minimum width=4.25cm, minimum height=3.75cm, yshift=-0.85cm,orange] (itinerary) {};

    \node[minimum width=4.35cm, minimum height=0.65cm, yshift=-0.55cm,blue] (row) {};

    \node[minimum width=1.1cm, minimum height=3.85cm, xshift=-0.525cm, yshift=-0.85cm, green] (column) {};

    \node[minimum width=0.95cm, minimum height=0.55cm, xshift=-0.525cm, yshift=-0.55cm, red] (cell) {};
  \end{tikzpicture}
  \caption{A document along with regions.}
\end{figure}

\end{comment}

\begin{algorithm}
\small
\caption{Synthesize Extraction Program}
\begin{algorithmic}[1]
\State \SynthesizeExtractionProgram ($C, m, \LL_{rg}, \LL_{ex}$)
\Require Cluster $C$, with annotations $\annotation(.)$ for a field $f_T$ 
\Require Landmark value $m$
\Require DSL $\LL_{rg}$
\Require DSL $\LL_{ex}$
\State $\mathsf{RegionSpec}  \gets \langle \rangle$ 
\State $\mathsf{ExtractionSpec} \gets \langle \rangle$ 
\State for each $ d_i \in C$
\State \quad $\ell^m \gets \locate(d_i, m)$
\State \quad $(L, a) \gets \annotation(d_i)$
\State \quad $\mathsf{RegionSpec} \gets
\mathsf{RegionSpec} + \langle (d_i, \ell^m),  \encr([\ell^m] \cup L, d) \rangle$
\State $P_{rg} \gets \mathsf{LearnRegionProgram}(\mathsf{RegionSpec}, \LL_{rg})$

\State $f \gets $ most commom blueprint of regions in $\mathsf{RegionSpec}$

\State for each $d_i \in C$
\State \quad $\ell^m \gets \locate(d_i, m)$
\State \quad $([\ell_1, \ell_2, \ldots, \ell_n], a) \gets \annotation(d_i)$
\State \quad $v \gets a(d_i[\ell_1], d_i[\ell_2], \ldots d_i[\ell_n])$
\State \quad $\mathsf{region} \gets P_{rg}(d_i, \ell^m)$
\State \quad $\mathsf{ExtractionSpec} \gets \mathsf{ExtractionSpec} + \langle \mathsf{region}, v \rangle$
\State $P_{ex} \gets \mathsf{LearnExtractionProgram}(\mathsf{ExtractionSpec}, \LL_{ex})$
\State \Return ($P_{rg}, f, P_{ex}$)
\end{algorithmic}
\end{algorithm}


More precisely, we are given a set of documents $C$ belonging to one cluster
with annotations $\annotation(d)$ for each $d \in C$ for a field $f_T$.  We also
assume that we are given a landmark value $m$ for the cluster, whose location is
"close" to the locations of the desired field value $f_T$ for all  $d \in C$.

 For each $d \in C$, let $\ell^m_d = \locate(d,m)$ be the location of the
 landmark $m$ in $d$, and let $[\ell^1_d, \ell^2_d, \ldots, \ell^n_d]$ be the
 locations in the annotation $\annotation(d)$ for the field value $f_T$.
 In all real-world data sets we have encountered, we have observed the following
 property: for a well-chosen landmark $m$, we have that (1) the location of the
 landmark,  is "close" to the locations of the field values, and (2) the
 "sub-region" of the document that contains the  landmark and the field values
 has identical structure for all documents $d \in \dtr$.
 Motivated by this property, we synthesize an extraction program $P$ such that
 $P(d)$ extracts the desired value $f_T(d)$ for not only all documents $d \in
 C$, but also robustly for unseen documents $\hat{d} \not \in C$ such that the
 sub-region of the document containing landmark and field values in $\hat{d}$
 has identical structure to documents in $C$
 


More precisely, the program $P$ we synthesize is a composition of two programs:
(1) a region growing  program $P_{rg}$, which takes the landmark $m$ as input
and produces a region $R_d$ (containing the sub-region of the document with
landmark and field values) as output, and (2) an extraction program $P_{ex}$
which takes the region $R_d$ produced by $P_{rg}$ as input, and extracts the
field value $f_T(d)$ from $R_d$.

Our landmark-based program synthesis algorithm is shown in
Algorithm~\ref{algo:lrsyn}. In addition to the cluster $C$ of annotated input
documents and landmark value $m$, it takes two Domain Specific Languages
$\LL_{rg}$ and $\LL_{ex}$.
First, we accumulate a $\mathsf{RegionSpec}$ across the training documents in
the cluster $C$(see lines 4-7) .
For each document $d$, the $\mathsf{RegionSpec}$ consists of a the document and
landmark location as input and the desired output is a region containing the
locations of the landmark as well as all the field locations present in the
annotation $\annotation(d)$.  The $\mathsf{LearnRegionProgram}$ function takes
this $\mathsf{RegionSpec}$ as input along with a DSL $\LL_{rg}$ to synthesize a
region program. The region program $P_{rg}$ takes the document and landmark
location as inputs and outputs a \emph{small} region around the landmark. 
In line 9, we calculate the most commonly occurring blueprint of all regions
in $\mathsf{RegionSpec}$. This value is used during execution of the synthesized
extraction program to make sure that the format of the region at extraction time
matches with the format of the region at synthesis time.

Next, we accumulate an $\mathsf{ExtractionSpec}$ across the training documents
(see lines 10-15) .
For each document $d$, the $\mathsf{ExtractionSpec}$ consists of the region
$P_{rg}(d)$ as input, and the field value as the desired output. The
$\mathsf{LearnExtractionProgram}$ function takes this $\mathsf{ExtractionSpec}$
as input along with a DSL $\LL_{ex}$ to synthesize an extraction program. An
extraction program $P_{ex}$ takes the document as input and outputs the desired
field value.

\section{Synthesis}
\begin{itemize}
    \item Provide dsls here
\end{itemize}
\spsays{TODO. Copied this segment from HDEF paper, revise it appropriately}
Mention cover loop

\paragraph{The HTML Extraction DSL}
The DSL $\LL_{ex}$ we use for the M2H email data-set is a combination of the
HTML extraction DSL from~\cite{} and the \textsc{FlashFill}
text-transformation DSL~\cite{}.
We do not explain the semantics of the DSL in detail, but instead
refer to the corresponding papers.
Informally, we use the HTML extraction DSL to select a set of DOM nodes
from each email, and then use the \textsc{FlashFill} DSL to transform the
text inside the DOM nodes to the field values.
The HTML extraction DSL is inspired by CSS selectors and each program is a 
composition of atomic selectors that act as filters on the set of DOM nodes
in the email.
The \textsf{FlashFill} DSL extracts sub-strings based on regular expression
matches within the text content of each DOM node.

\begin{comment}
\subsection{Evaluation on FX DS3 dataset}
We also evaluate $\ndsyn$ and $\resyn$ on the DS3 dataset published by $\textsf{ForgivingXPaths}$ authors. The dataset primarily consists of product web pages across $k$ different providers. For our experiments, we sample $15$ web pages uniformaly at random from this dataset as our train data and evaluate on the remaining data, for each provider. We do $5$ runs of this experiment with different train samples and report the average numbers.

Table~\ref{} shows the F1 scores for $\ndsyn$ and $\resyn$ on this dataset. As seen from this experiment, \spsays{TODO}

\end{comment}
\begin{comment}
To that effect, we further split the test data into two parts: one comprising of emails which are consistent with the landmarks and blueprints, and other consisting of emails which are not consistent. Table~\ref{}~indicates the proportion of this split. As we can see from the table, the number of emails which are not consistent is fairly less, even though the test data was gathered from a different time period. This also points that narrowing down to small regions helps, as the core regions do not change often in datasets. In this experiment, we perform our comparison only with test emails which are consistent with the training data for that domain. We discuss more about the remaining emails in the next section.
\end{comment}



\begin{comment}
\begin{table}
\small
\label{table:m2hexpmt_1}
\begin{tabular}{|c|l|c|c|c|}
\hline
{Domain} & Fields & $\textsf{FX}$ & $\ndsyn$ & $\resyn$\\
\hline
\hline\multirow{9}{*}{itinerary.westjet}

& AIata &  &  1.00 & 1.00 \\
& ATime &  &  1.00 & 1.00 \\
& DIata &  &  1.00 & 1.00 \\
& DDate &  &  1.00 & 1.00 \\
& DTime &  &  1.00 & 1.00 \\
& FNo   &  &  1.00 & 1.00 \\
& Name  &  &  1.00 & 1.00 \\
& Pvdr  &  &  1.00 & 1.00 \\
& RId   &  &  1.00 & 1.00 \\

\hline\multirow{9}{*}{aeromexico}

& AIata &  &  1.00 & 1.00 \\
& ATime &  &  1.00 & 1.00 \\
& DIata &  &  1.00 & 1.00 \\
& DDate &  &  1.00 & 1.00 \\
& DTime &  &  1.00 & 1.00 \\
& FNo   &  &  1.00 & 1.00 \\
& Name  &  &  1.00 & 1.00 \\
& Pvdr  &  &  1.00 & 1.00 \\
& RId   &  &  1.00 & 1.00 \\

\hline\multirow{9}{*}{mytrips.amexgbt}
& AIata &  &  1.00 & 1.00 \\
& ATime &  &  0.99 & 1.00 \\
& DIata &  &  1.00 & 1.00 \\
& DDate &  &  0.99 & 1.00 \\
& DTime &  &  1.00 & 1.00 \\
& FNo   &  &  1.00 & 1.00 \\
& Name  &  &  1.00 & 1.00 \\
& Pvdr  &  &  1.00 & 1.00 \\
& RId   &  &  1.00 & 1.00 \\

\hline\multirow{9}{*}{qatarairways.com.qa}

& AIata &  &  1.00 & 1.00 \\
& ATime &  &  0.99 & 1.00 \\
& DIata &  &  1.00 & 1.00 \\
& DDate &  &  0.99 & 1.00 \\
& DTime &  &  1.00 & 1.00 \\
& FNo   &  &  1.00 & 1.00 \\
& Name  &  &  1.00 & 1.00 \\
& Pvdr  &  &  1.00 & 1.00 \\
& RId   &  &  0.99 & 1.00 \\

\hline
\end{tabular}
\end{table}
\end{comment}

\begin{comment}
\subsubsection{Inconsistent test emails}
In this experiment, we evaluate on test emails which were not consistent with train emails with respect to landmarks and blueprints. In the M2H dataset, there were only $4$ domains which had inconsistent emails. All these emails were marked inconsistent because the blueprints did not match owing to a different structure, though the landmark remained the same. If we group these outlier emails based on blueprints inferred using ground truth, delta.com had $k$ groups, Philippines had $k2$ groups, qatar had $k3$ and alaksa had $k4$ groups.
 
There are various ways we can deal with this issue. We can use NDSyn programs or a ML model to predict on these emails and add the labelled set to the training data. In this work, we adopt a simpler method: We sample some emails from this set and add it to the training data. Table~\ref{}~shows the performance once more emails are added to the training data.

Interesting example where landmark improved on addition of new data.
\end{comment}

We treat the \emph{n-grams} appearing across all the HTML documents as landmark
candidates. We filter candidates which appear in our stop word file, like
punctuation and pronouns. We also filter n-grams which are very lengthy.  Given
a landmark candidate and a document, field values (which are obtained from the
annotations) We use two types of scores:
\begin{enumerate}
    \item We render the HTML document in a browser and find the sum of Euclidean distance between the landmark location and the field value locations. The intuition here is that a \emph{good} landmark candidate will appear very close to the field values in all the documents.
    \item Given the landmark location and the field regions, we use the $\mathsf{LearnRegionProgram}$ routine to compute the enclosing region. And we measure the region size by the number of nodes in this region. The main reasoning here is that a smaller region will have lesser number of nodes in practice.
\end{enumerate}
The final score is a sum of these two scores weighted appropriately for scale.
In our ablation experiments, we also experiment with other scoring measures like
Manhattan distance and left-aligned scores. 

\subsubsection{$\mathsf{LearnRegionProgram}$ and Blueprints for HTML documents}
The goal of $\mathsf{LearnRegionProgram}$ function is to find a \emph{small}
enclosing region given a pair of landmark and field values $\langle \ell^m_d,
\ell^{f_T}_d \rangle$. For simplicity, let us assume that there is $1:n$ between
the landmark and field values. We will describe the generalization to the $m:n$
case later.

An HTML document provides an explicit tree structure which we leverage to find
the smallest enclosing region given a landmark and field value. Intuitively, the
encompassing smallest region will be a sibling region or the lowest common
ancestor (LCA) of landmark and the field values. We represent $P_{rg}$ using
$\mathsf{parentHops}, \mathsf{siblingHops}$ such that they cover all the train
documents. We omit the detailed procedure computing these hops and refer the
readers to the Appendix.

\paragraph{$\mathsf{Blueprint}$ for a HTML web region} HTML document provides
us with an explicit tree structure. For computing a blueprint for an input web
region, we gather a sequence of tags in terms of their XPaths from a
$\mathsf{PreordeTraversal}$ starting from the begin node and ending at the last
node of the region. We ignore the indexes in the \spsays{Add more nuances here,
we filter out similar tag structures} %For instance, tr\\td\\tr\\td \to tr\\td}.


We first process structured images using Optical Character Recognition (OCR)
packages~\cite{ocr1,ocr2}, which returns a list of bounding boxes and their
associated texts. Like in HTML, we treat bounding boxes which appear very close
to each other as \emph{n-grams}. We gather the \emph{n-grams} appearing across
all the structured images as landmark candidates.  For scoring the landmark, we
again employ two scores as below. Unlike HTML which requires rendering, the
bounding boxes here directly give us the visual coordinates.

\begin{enumerate}
    \item We find the sum of Euclidean distance between the landmark region and the field regions. We use the center of these regions to compute the distances.
    \item We also measure the size of the rectangle induced by the landmark region and the field region.
\end{enumerate}
The final score is a sum of these two scores weighted appropriately for scale.


\begin{comment}
\begin{algorithm}
\small
\caption{$\mathsf{Blueprint}$ for a HTML web region}
\label{algo:blueprint}
\begin{algorithmic}[1]
\Require HTML web region $R$
\State $\mathsf{BluePrint} \gets \mathsf{TagSequence}$ of $\mathsf{PreordeTraversal}$ from the start of web region to end of web region
\State \Return $\mathsf{BluePrint}$
\end{algorithmic}
\end{algorithm}
\end{comment}

\spsays{Rough first draft}
As a first step, we do an OCR on structured images which returns bounding boxes and associated text. As we do not have explicit tag structure like HTML, the region program on top of OCR boxes is more complex. Recall that the goal of $\mathsf{LearnRegionProgram}$ is to find/enumerate region(s) satisfying the $\encr$ property. Additionally, we want the outputted region to be as small as possible. 

Figure~\ref{}~depicts the overall idea behind the region growing algorithm for images. Given an initial $\mathsf{region}$, we can expand it in all directions so as to find an enclosing region. Specifically, we start with the landmark region as in HTML, and we would like to expand this region to encompass all the field regions. We expand in any direction only if required. To control the expansion, we leverage the following properties:
\begin{enumerate}
    \item If we know the field pattern, then we can continue expanding till we find this pattern. $\mathsf{Expand(Bottom, fieldpattern)}$
    \item We can continue expanding till we hit a boundary pattern, which we can choose to include or exclude. $\mathsf{Expand(Right, pattern, include/exclude)}$
    \item We can expand in an absolute manner. For instance, $\mathsf{Expand(Left, 1)}$
\end{enumerate}

\begin{example}
Figure~\ref{}~depicts the region growing procedure for an accounts invoice, for various fields.
\begin{itemize}
    \item If we want to extract the document date given $\mathsf{Date}$ as a landmark, we can Expand one region to the right and extract the value. We can also keep expanding the region till a Date type is found.
    \item Likewise, if we want to extract account number, given $\mathsf{Account No.}$ as landmark, we can expand one region to the bottom and extract the value.
    \item Extracting the chassis value is more complex, as it can contain varied number of tokens and might not abide to a strict field pattern. In this case, we traverse one region down and keep expanding to the right until we hit the engine value pattern, which we do exclude from this region.
    \item Extracting customer address or invoice address requires us to keep traversing in the downwards direction and collecting all the lines until we hit a pattern like zip code or a stopping criterion like the constant \emph{Raised by} or \emph{Invoiced by}. 
\end{itemize}
\end{example}

\begin{verbatim}
language Visual;
feature double Score = Microsoft.ProgramSynthesis.Extraction.Forms.Learning.RankingScore;

@start List<Region> roi := landmarks | bothDirections;
List<Region> bothDirections := ExtendLineItems(roi, pattern)
										| ExtendAbsAbs(roi, axis, k, k)
										| ExtendAbsRel(roi, axis, k, pattern, isIncl)
										| ExtendRelAbs(roi, axis, pattern, isIncl, k)
										| ExtendRelRel(roi, axis, pattern, isIncl, pattern, isIncl);

int k;
Axis axis;
RegexToken pattern;
bool isIncl;

@input List<Region> landmarks;
\end{verbatim}

\begin{comment}
\begin{figure}
\small
\begin{tabular}{r c l}
regionProg & := & $\;\;$\textsf{landmarks} \\
          &    & | \textsf{ExtendAbsAbs}(\textit{regionProg}, \textit{axis}, \textit{k}, \\
          &    & \textit{k}) \\
          &    & | \textsf{ExtendAbsRel}(\textit{regionProg}, \textit{axis}, \textit{k}\\
          &    & \textit{pattern}, \textit{isIncl}) \\
          &    & | \textsf{ExtendRelAbs}(\textit{regionProg}, \textit{axis}, \\
          &    & \textit{pattern}, \textit{incl}, \textit{k}) \\
          &    & | \textsf{ExtendRelRel}(\textit{regionProg}, \textit{axis}, \\
          &    & \textit{pattern}, \textit{isIncl}, \textit{pattern}, \textit{isIncl}) \\
\end{tabular}
\textit{axis} $\in$ $\langle Up, Down, Left, Right \rangle$; Set[Pattern] \textit{pattern};
\vspace{-2ex}
\caption{Syntax of the visual region-growing language $\LL_{rg}$}
\label{fig:visual-dsl}
\end{figure}
\end{comment}

\paragraph{Talk about enumerative synthesis}
Figure~\ref{fig:visual-dsl} describes the region DSL $\L_{rg}$ for images. Starting from an initial landmark region, we have two broad cases:
\begin{compactitem}
\item The landmark region itself encompasses all the fields, in which case the $\textsf{regionProg}$ just returns the landmark region
\item We expand the landmark region in such a way that we enclose the field regions. The expansion can be done along all four cardinal directions. We group the left-right as one group and top-down as another group. In each of this group, we can either expand in an \emph{absolute} sense or in a \emph{relative} way.  
\end{compactitem}

\paragraph{Cover loop in region growing}
In HTML, we could find the enclosing region with parent and sibling hops. In images, we grow the region  using Enumerative synthesis with the DSL shown above. To account for the variability in the images and the resulting OCR, we employ a cover loop to find a disjunction of programs to cover the training data, instead of a single program.

\spsays{Give example}
\spsays{Give cover loop pseudo code}
\spsays{Move all blueprinting logic to clustering?}

\subsubsection{Blueprints for images} Images do not provide an explicit tag structure which we can use for blueprints, unlike HTML. As first step, we compute a frequency histogram of n-grams occurring in the given input images. Recall that, we first perform an OCR on the input image which provides us with bounding boxes and their corresponding text. We retain the top $k\%$ of the frequently occurring n-grams as the tags for images. Our goal is to describe a given input document with respect to these tags.

For doing so, we compute the neighborhood information for each tag in the $4$ cardinal directions. The neighbors for a given tag are close-by elements, and can either be another frequently occurring n-gram or a variable text. If it turns out to be a variable text, we denote the existence of the box, rather than a specific n-gram. So the given image in Figure~\ref{fig:formsextraction}~can be described in terms of these tags as $\langle <VatRegNo><Top>NIL</Top><Right>NIL></Right><Bottom>Exists</Bottom><Right>Nil></Right> </VatRegNo><InvoiceTo>...$ and so on. \spsays{Need a better forms example}. Section~\ref{}~provides more details on how we use BluePrints during clustering and inference.

\begin{theorem}
Given $\mathsf{LearnRegionProgram}$ for an input domain, the synthesized program $\P$ is robust to any changes occurring outside of the enclosed region.
\end{theorem}


\begin{comment}
\begin{table*}[t]
\small
\label{table:m2hexpmt2}
\resizebox{15cm}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
{Domain} & \multicolumn{2}{|c|}{ArrivalAirportIata} &\multicolumn{2}{|c|}{ArrivalTime} & \multicolumn{2}{|c|}{DepartureAirportIata} &\multicolumn{2}{|c|}{DepartureDate} &\multicolumn{2}{|c|}{DepartureTime} \\
\cline{2-11} &  RobustLmk & UserLmk & RobustLmk & UserLmk & RobustLmk & UserLmk & RobustLmk & UserLmk & RobustLmk & UserLmk \\

\hline\multirow{2}{*}{ifly.alaskaair.com}
&Arrives&Arrives&Arrives&Arrives&Departs&Departs&Departs&Departs&Departs&Departs\\
&&&&&&&Confirmation code: $->$Term/Gate&Term Gate&&\\
\hline\multirow{2}{*}{delta.com}
&Departure Time&To&Arrival Time&Arrival Time&Flight&From&Departure Time&Departure Time&Departure Time&Departure Time\\
&Flight Number:&Arrives&Arrives&Arrives&Departs&Departs&Departs&Departs&Departs&Departs\\
\hline\multirow{1}{*}{booking.airasia.com}
Arrive&Arrive&Arrive&Arrive&Depart&Depart&Depart&Depart&Depart&Depart&Depart\\
\hline\multirow{1}{*}{getthere.com}
&Arrive:&Arrive:&Arrive:&Arrive:&Depart:&Depart:&Depart:&Depart:&Depart:&Depart: \\
\hline\multirow{1}{*}{t.delta.com}
&ARRIVE&ARRIVE&ARRIVE&ARRIVE&DEPART&DEPART&DEPART&DEPART&DEPART&DEPART\\
\hline\multirow{2}{*}{philippineairlines.com}
&Departure&To&Arrival&Arrival&New&From&Departure&Departure&Departure&Departure\\
&Philippine Airlines&Outbound&Philippine Airlines&Outbound&Outbound&Outbound&Family:->Fare&Outbound&Philippine Airlines&Outbound\\
\hline\multirow{1}{*}{itinerary.westjet.com}
&Arrival:&Arrival:&Arrival:&Arrival:&Departure:&Departure:&Flight Number&Flight Number&Departure:&Departure:\\
\hline\multirow{1}{*}{aeromexico.com}
&Route&Route&Arrives&Arrives&Route&Route&Date&Date&Departs&Departs\\
\hline\multirow{1}{*}{mytrips.amexgbt.com}
&Destination:&Destination:&Arriving:&Arriving:&Origin:&Origin:&Departing:&Departing:&Departing:&Departing:\\
\hline\multirow{1}{*}{qatarairways.com.qa}
&Arrival&Arrival&Arrival&Arrival&Departure&Departure&Arrival&Arrival&Departure&Departure\\
\hline
\end{tabular}
}
\caption{Landmarks detected vs User Selected Landmarks}
\end{table*}

\begin{table*}
\small
\label{table:m2hexpmt2}
\resizebox{15cm}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
{Domain} & \multicolumn{2}{|c|}{FlightNumber} &\multicolumn{2}{|c|}{Name} & \multicolumn{2}{|c|}{Provider} &\multicolumn{2}{|c|}{ReservationId} \\
\cline{2-9} &  RobustLmk & UserLmk & RobustLmk & UserLmk & RobustLmk & UserLmk & RobustLmk & UserLmk \\

\hline\multirow{1}{*}{ifly.alaskaair.com}
&Departs&Flight&Travelers:&Travellers&&&Travelers:->Confirmation code:&ConfirmationCode\\
\hline\multirow{2}{*}{delta.com}
&Flight&Flight&Name&Name&Carrier&Carrier&Flight Information (Record Locator :&Flight Information (Record Locator : \\
&Flight Number:&Flight Number:&Who's Coming Along&Who's Coming Along&Flight Number:&Flight Number:&Confirmation Number :&Confirmation Number : \\
\hline\multirow{1}{*}{booking.airasia.com}
&Depart&Depart&Guests&Guests&Depart&Depart&Booking number&Booking number\\

\hline\multirow{1}{*}{getthere.com}
&Flight/Equip&Flight/Equip&Meal:->Name:&Name&Flight/Equip&Flight/Equip&Airline Record Locator&Airline Record Locator\\
\hline\multirow{2}{*}{t.delta.com}
&DEPART&DEPART&Name:&Name:&DEPART&DEPART&Confirmation \#:&Confirmation \#: \\
&&&&&&&Your Trip Confirmation \#:&Your Trip Confirmation \#: \\
\hline\multirow{2}{*}{philippineairlines.com}
&Flight&Flight&Dear&Dear&Flight&Flight&Booking reference:&Booking reference:\\
&Philippine Airlines&Philippine Airlines&Passengers&Passengers&Philippine Airlines&Philippine Airlines&Reference:&Reference:\\
\hline\multirow{1}{*}{itinerary.westjet.com}
&Flight Number->WESTJET&Flight Number&Seat(s):&Seat(s):&Flight Number->WESTJET&WESTJET&WestJet&WestJet\\
\hline\multirow{1}{*}{aeromexico.com}
&Flt \#&Flt \#&Passengers&Passengers&Flt \#&Flt \#&Confirmation Code:&Confirmation Code:\\
\hline\multirow{1}{*}{mytrips.amexgbt.com}
&Flight:&Flight:&Booking Reference:&Traveler&Flight:&Flight:&Airline Booking Ref:&Airline Booking Ref:\\
\hline\multirow{2}{*}{qatarairways.com.qa}
&Class&Class&Passenger name/ E&Passenger name&Class&Class&Booking reference (PNR)&Booking reference (PNR)\\
&Class&Class&&&Class&Class&Booking reference (PNR)&Booking reference (PNR)\\
\hline
\end{tabular}
}
\caption{Landmarks detected vs User Selected Landmarks}
\end{table*}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table*}[t]
\small
\label{table:m2hexpmt1}
\begin{tabular}{|c|c|c|c||c|c|c|c|c|c|c|c|c|}
\hline
 \multirow{\shortstack[c]{Domain}} & \multirow{Fields} & \multicolumn{4}{|c|}{NDSyn} & \multicolumn{4}{|c|}{$\hisyn$}\\
\cline{3-19}&  & #Programs & Pre. & Rec. & F1 & #Programs & Pre. & Rec. & F1\\
\hline
\hline\multiline{ifly.alaskaair.com}
& ArrivalAirportIata & 2 & 0.9989 & 0.4718 & 0.6409 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
& ArrivalTime & 2 & 0.9697 & 0.4576 & 0.6218 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
& DepartureAirportIata&2&0.8888&0.4198&0.5703&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00 \\
& DepartureDate&1&1.00&1.00&1.00&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00 \\
& DepartureTime&2&0.8989&0.4241&0.5763&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00 \\
& FlightNumber&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\ 
& Name&1&1.00&0.9751&0.9874&1&1&1.00&0.9751&0.9874&0& & & & &1.00&0.9751&0.9874\\ 
& ReservationId&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
\hline\multiline{delta.com}
& ArrivalAirportIata&2&0.9967&0.9967&0.9967&2&2&1.00&1.00&1.00&7&2&0.0000&0.0000&0.0000&0.9967&0.9967&0.9967\\
& ArrivalTime&2&0.9962&0.9975&0.9968&2&2&1.00&1.00&1.00&7&2&0.0000&0.0000&0.0000&0.9962&0.9975&0.9968\\
& DepartureAirportIata&2&0.9934&0.9967&0.9950&2&2&0.9934&0.9967&0.9950&0& & & & &0.9934&0.9967&0.9950\\
& DepartureDate&1&0.9320&0.9659&0.9486&2&2&1.00&1.00&1.00&7&1&0.1429&0.3636&0.2052&0.9951&0.9986&0.9968\\
& DepartureTime&2&1.00&0.9975&0.9987&2&2&1.00&1.00&1.00&7&2&0.0000&0.0000&0.0000&1.00&0.9975&0.9987\\
& FlightNumber&2&1.00&1.00&1.00&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Name&2&0.9447&0.8795&0.9109&2&2&0.9508&1.00&0.9748&7&2&0.0000&0.0000&0.0000&0.9508&0.9951&0.9724\\
& Provider&2&1.00&1.00&1.00&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ReservationId&2&1.00&0.9915&0.9957&2&2&1.00&0.9989&0.9994&8&2&1.00&0.2222&0.3636&1.00&0.9915&0.9957\\
\hline\multiline{booking.airasia.com}
& ArrivalAirportIata&1&0.5000&1.00&0.6667&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ArrivalTime&0& NaN&0.0000&0.0000&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureAirportIata&1&0.5000&1.00&0.6667&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureDate&1&0.5000&1.00&0.6667&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureTime&0& NaN&0.0000&0.0000&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& FlightNumber&1&1.00&0.8974&0.9459&1&1&1.00&0.9189&0.9577&1&1&1.00&0.5000&0.6667&1.00&0.8974&0.9459\\
& Name&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Provider&1&1.00&0.8974&0.9459&1&1&1.00&0.9189&0.9577&1&1&1.00&0.5000&0.6667&1.00&0.8974&0.9459\\
& ReservationId&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
\hline\multiline{getthere.com}
& ArrivalAirportIata&3&0.7356&0.8384&0.7836&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ArrivalTime&2&0.9384&0.9114&0.9247&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureAirportIata&3&0.9426&0.9452&0.9439&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureDate&3&0.9834&0.9378&0.9601&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureTime&2&0.8659&0.8619&0.8639&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& FlightNumber&1&0.9409&0.9589&0.9498&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Name&1&0.8285&0.9641&0.8912&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Provider&1&0.9804&0.9530&0.9665&1&1&1.00&1.00&1.00&1&1&0.0000&0.0000&0.0000&1.00&1.00&1.00\\
& ReservationId&1&1.00&0.8757&0.9337&1&1&1.00&1.00&1.00&1&1&0.0000&0.0000&0.0000&1.00&0.9941&0.9970\\
\hline\multiline{t.delta.com}
& ArrivalAirportIata&1&0.9996&0.9979&0.9987&1&1&1.00&0.9982&0.9991&2&1&0.9231&0.9231&0.9231&0.9996&0.9979&0.9987\\
& ArrivalTime&1&0.9978&1.00&0.9989&1&1&0.9982&1.00&0.9991&2&1&0.9231&1.00&0.9600&0.9978&1.00&0.9989\\
& DepartureAirportIata&1&1.00&0.9986&0.9993&1&1&1.00&0.9986&0.9993&2&1&1.00&1.00&1.00&1.00&0.9986&0.9993\\
& DepartureDate&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureTime&1&0.9975&1.00&0.9987&1&1&0.9975&1.00&0.9987&2&1&1.00&1.00&1.00&0.9975&1.00&0.9987\\
& FlightNumber&2&1.00&0.9634&0.9814&1&2&1.00&0.9687&0.9841&2&2&1.00&1.00&1.00&1.00&0.9688&0.9842\\
& Name&1&0.9976&0.9976&0.9976&1&1&0.9976&0.9976&0.9976&63&1&0.0000&0.0000&0.0000&0.9976&0.9976&0.9976\\
& Provider&2&0.9928&0.9400&0.9657&1&2&1.00&0.9472&0.9729&2&2&1.00&0.6250&0.7692&1.00&0.9453&0.9719\\
& ReservationId&1&1.00&1.00&1.00&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
\hline\multiline{alaskaair.com}
& ArrivalAirportIata&2&1.00&1.00&1.00&6&5&1.00&0.9990&0.9995&27&2&1.00&1.00&1.00&1.00&0.9990&0.9995\\
& ArrivalTime&2&1.00&1.00&1.00&6&5&1.00&0.9990&0.9995&27&2&1.00&1.00&1.00&1.00&0.9990&0.9995\\
& DepartureAirportIata&2&1.00&1.00&1.00&6&5&1.00&0.9990&0.9995&27&2&1.00&1.00&1.00&1.00&0.9990&0.9995\\
& DepartureDate&2&1.00&0.9997&0.9998&6&3&1.00&0.9948&0.9974&38&2&1.00&0.9932&0.9966&1.00&0.9948&0.9974\\
& DepartureTime&2&1.00&1.00&1.00&6&5&1.00&0.9990&0.9995&27&2&1.00&1.00&1.00&1.00&0.9990&0.9995\\
& FlightNumber&1&0.9603&0.9995&0.9795&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Name&2&1.00&1.00&1.00&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Provider&2&1.00&0.9644&0.9819&2&2&1.00&0.9767&0.9882&5&2&1.00&0.5333&0.6956&1.00&0.9735&0.9866\\
& ReservationId&2&1.00&1.00&1.00&2&2&1.00&1.00&1.00&165&2&1.00&1.00&1.00&1.00&1.00&1.00\\
\hline\multiline{philippineairlines.com}
& ArrivalAirportIata&3&0.9191&1.00&0.9578&2&3&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ArrivalTime&2&1.00&1.00&1.00&2&3&1.00&0.9811&0.9905&0& & & & &1.00&0.9811&0.9905\\
& DepartureAirportIata&2&0.9937&0.9937&0.9937&2&2&0.9932&0.9932&0.9932&5&2&1.00&1.00&1.00&0.9937&0.9937&0.9937\\
& DepartureDate&2&0.9815&0.9463&0.9636&2&2&0.9815&0.9463&0.9636&0& & & & &0.9815&0.9463&0.9636\\
& DepartureTime&2&1.00&1.00&1.00&2&3&1.00&0.9811&0.9905&0& & & & &1.00&0.9811&0.9905\\
& FlightNumber&3&0.7397&0.6792&0.7082&2&3&1.00&0.9308&0.9642&0& & & & &1.00&0.9308&0.9642\\
& Name&3&1.00&0.9745&0.9871&2&2&1.00&0.9954&0.9977&0& & & & &1.00&0.9954&0.9977\\
& Provider&2&1.00&1.00&1.00&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ReservationId&2&1.00&1.00&1.00&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
\hline\multiline{itinerary.westjet.com}
& ArrivalAirportIata&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ArrivalTime&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureAirportIata&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureDate&1&1.00&0.9956&0.9978&1&1&1.00&1.00&1.00&73&1&1.00&0.9757&0.9877&1.00&0.9956&0.9978\\
& DepartureTime&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& FlightNumber&1&1.00&1.00&1.00&1&1&1.00&0.9965&0.9982&0& & & & &1.00&0.9965&0.9982\\
& Name&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&73&1&1.00&1.00&1.00&1.00&1.00&1.00\\
& Provider&1&1.00&1.00&1.00&1&1&1.00&0.9965&0.9982&0& & & & &1.00&0.9965&0.9982\\
& ReservationId&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
\hline\multiline{aeromexico.com}
& ArrivalAirportIata&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ArrivalTime&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureAirportIata&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureDate&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureTime&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& FlightNumber&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Name&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Provider&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
\hline\multiline{mytrips.amexgbt.com}
& ReservationId&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ArrivalAirportIata&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ArrivalTime&1&0.9948&1.00&0.9974&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureAirportIata&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureDate&1&0.9955&1.00&0.9977&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& DepartureTime&1&0.9955&1.00&0.9977&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& FlightNumber&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Name&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& Provider&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
& ReservationId&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
\hline\multiline{qatarairways.com.qa}
& ArrivalAirportIata&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&20&1&1.00&1.00&1.00&1.00&1.00&1.00\\
& ArrivalTime&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&20&1&1.00&1.00&1.00&1.00&1.00&1.00\\
& DepartureAirportIata&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&20&1&1.00&1.00&1.00&1.00&1.00&1.00\\
& DepartureDate&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&20&1&1.00&1.00&1.00&1.00&1.00&1.00\\
& DepartureTime&1&1.00&1.00&1.00&1&1&1.00&1.00&1.00&20&1&1.00&1.00&1.00&1.00&1.00&1.00\\
& FlightNumber&1&0.9982&1.00&0.9991&2&1&0.9981&1.00&0.9990&20&1&1.00&1.00&1.00&0.9982&1.00&0.9991\\
& Name&1&0.9988&1.00&0.9994&1&1&0.9988&1.00&0.9994&0& & & & &0.9988&1.00&0.9994\\
& Provider&1&1.00&1.00&1.00&2&1&1.00&1.00&1.00&20&1&1.00&1.00&1.00&1.00&1.00&1.00\\
& ReservationId&2&1.00&0.9967&0.9983&2&2&1.00&1.00&1.00&0& & & & &1.00&1.00&1.00\\
\hline
\end{tabular}
\caption{#Program, Precision, Recall and F1 numbers on HTML extraction scenario (M2H dataset) with NDSyn and $\hisyn$}
\end{table*}

\end{comment}

\begin{comment}
\item FX Dataset
    \begin{itemize}
    \item Description: E-commerce website product pages from 4 domains(bestbuy, currys, ebuyer and pricerunner).
    \item Methodology:
    Out of the 1000 emails provided for each domain, we first cleaned the dataset to remove pages where there were annotations missing for a given field. After this, 150 pages were sampled randomly from the now cleaned dataset to create training sets. We further considered 5 seeds to randomly sample our trainsets. The trainsets sampled were of sizes 5, 10, 15 and 20 pages. The remaining pages were used as the test set to calculate the following metrics. 
    \item Metrics: Precision, Recall, F1 score, \#Programs, Method of landmark scoring, \#NotInCluster
    \end{itemize}
\end{comment}

\spsays{TODO}
\spsays{Write this formally}
\spsays{Give example? Should we add code for this, as we might run out of
space?}
Landmark values can occur at multiple places in a given document. Our aim is to
narrow down the region precisely. We proceed as follows:
\begin{enumerate}
    \item We grow the region around the landmark and field values. And compute
    the blueprint of this small region. We also use this region program to
    grow the region around other occurrences of this same landmark value. And
    compute the blueprints of these regions. If the blueprints differ, then
    we are done. We already have a disambiguating <landmark, blueprint> pair.
    \item If the <landmark, blueprint> is ambiguous, we learn one more level
    of hierarchy. For this, we treat the current landmark value as a field, and
    learn a landmark for this value.
    \item We repeat this procedure till we find a disambiguating <landmark,
    blueprint> pair.
\end{enumerate}

At inference time, we locate the topmost landmark value in the hierarchy, in the
given document. Then we locate the next nearest landmark value and so on till we
locate the last value of the landmark. Then we use the region program to grow
the regions, match the blueprints and run extraction program on each of these
regions. 

\begin{figure*}[th]
\centering
\begin{minipage}{5cm}
\includegraphics[width=5cm]{images/forms_regiongrowing.png}
\label{fig:formsregion}
%\caption{}
\end{minipage}
\qquad
\begin{minipage}{7cm}
\frame{\includegraphics[width=9cm]{images/forms_image2_annotated.png}}
\label{fig:formsextraction2}
%\caption{}
\end{minipage}
\caption{Improve these images.Anonymize these images}
\end{figure*}



Our travel emails dataset is called the {\em machine-to-human (M2H)} dataset.
%
We perform two experiments with the M2H dataset: contemporary and longitudinal.
%
In the contemporary experiment, the training and test datasets contain
anonymized emails from the same time period.
%
In the longitudinal experiment, we evaluate our method with training and test
data across different time periods.
The M2H dataset consists of anonymized emails from $6$ different flight
providers. Each domain has  2 to 10 structural variations. We perform our
experiments one provider at a time. We synthesize programs for a given provider
with the training data and predict on the corresponding test data.
Table~\ref{table:m2hdataset}~shows the training and test data sizes for each
flight domain.

We compare the performance of \resyn~with two other approaches: (1) the \ndsyn~algorithm from prior work on heterogeneous data extraction~\cite{ij2019}, and (2) the \fx\ algorithm~\cite{omari2017synthesis}.
Our goal is to extract various fields from these varied data formats with an intention to answer the following questions:
\begin{compactitem}
\item \emph{Q1: How does $\resyn$ compare with previous approaches, namely $\ndsyn$ and $\textsf{ForgivingXPaths}$ in  contemporary and longitudinal settings?}
\item \emph{Q2: How do the automatically learnt landmarks by $\resyn$ compare to user provided landmarks?} 
\item \emph{Q3: How do the programs  synthesized by $\resyn$ and  $\ndsyn$ compare in terms of simplicity and robustness?}
\end{compactitem}

\begin{table}
\scriptsize
\begin{tabular}{|l|c|c|c|}
\hline
Domain & \shortstack[c]{Train \\ Size} & \shortstack[c]{Test \\ Size}\\
\hline
iflyalaskaair & 100 & 1092\\ \hline
delta & 102 & 928 \\ \hline
getthere & 50 & 154 \\ \hline
\end{tabular}
%
\hspace{3ex}
%
\begin{tabular}{|l|c|c|c|}
\hline
Domain & \shortstack[c]{Train \\ Size} & \shortstack[c]{Test \\ Size}\\
\hline
airasia & 25 & 24 \\ \hline
aeromexico & 35 & 303 \\ \hline
amex & 50 & 640 \\ \hline
\end{tabular}
\caption{M2H dataset}
\label{table:m2hdataset}
\vspace{-2ex}
\end{table}
%
\paragraph{Overall results}
Table~\ref{table:m2hoverall}~shows the average precision, recall and F1 scores across various extraction tasks for $\fx$, $\ndsyn$ and $\lrsyn$ for both contemporary and longitudinal setting. Unlike $\ndsyn$ or $\lrsyn$ which use a combination of structure and text programs for extraction, $\textsf{ForgivingXPaths}$ only outputs XPaths which correspond to the entire node, rather than the sub-text contained within that node. Consequently, $\textsf{ForgivingXPaths}$ has high recall and poor precision. We therefore omit $\textsf{ForgivingXPaths}$ from more detailed results tables below. We also observe that the gap between $\resyn$ and  $\ndsyn$, as measured by precision, recall (and thereby F1 score) is larger in the longitudinal evaluation as compared to the contemporary one. This is because programs synthesized by $\resyn$ generalize better and handle format changes better than $\ndsyn$.

\highlightbox{
$\lrsyn$ is very robust to variations in the longitudinal
setting, achieving $>95\%$ F1 score in all $53$ fields, with a perfect F1 score of $1.00$ in $49$ cases, as compared to $40$ and $33$ cases for $\ndsyn$.
}
%
In many applications, having a score of $1.00$ is crucial, i.e., even a system with $0.99$ 
precision cannot be deployed in practice.
%
For example, even a tiny imprecision in a system that automatically adds calendar entries
based on flight reservation emails is disastrous for millions of users.

\begin{table}
\scriptsize
\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{4}{|c|}{Contemporary} \\
\hline
Metric & $\fx$ & $\ndsyn$ & $\lrsyn$\\
\hline
Avg. Precision & 0.17 & 0.96 & 1.00\\ \hline
Avg. Recall & 0.99 & 0.91 & 1.00\\ \hline
Avg. F1 & 0.22 & 0.93 & 1.00 \\ \hline
\end{tabular}
\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{4}{|c|}{Longitudinal} \\
\hline
Metric & $\fx$ & $\ndsyn$ & $\lrsyn$\\
\hline
Avg. Precision & 0.15 & 0.99 & 1.00\\ \hline
Avg. Recall & 0.98 & 0.89 & 1.00\\ \hline
Avg. F1 & 0.20 & 0.92 & 1.00 \\ \hline
\end{tabular}
\caption{F1 scores for $\lrsyn$ and $\ndsyn$ for the M2H Contemporary and Longitudinal datasets}
\label{table:m2hoverall}
\end{table}


\paragraph{Detailed comparison}
Table~\ref{tab:m2hexpmt1} shows a more detailed drill-down of the F1 scores for $\ndsyn$ and $\resyn$, in the two settings. For a further drill-down of the F1 score into precision and recall, please see the supplementary material.
The rows of the table correspond to 53 extraction tasks, each corresponding to a field value, over the 6 airline domains in the M2H dataset. 
As seen from the table, $\lrsyn$ performs much better than $\ndsyn$ on 23 out of the 53 fields in the contemporary setting, and 24 out of 53 fields in the longitudinal setting. In the remaining fields, the two approaches have comparable F1 scores.

For the fields \emph{AIata}, \emph{ATime}, \emph{DIata} and \emph{DTime} in the \emph{iflyalaskaair} domain, we find that $\lrsyn$ performs much better than $\ndsyn$, and the gap between the two is wider in the longitudinal setting.
In the case of files \emph{ATime} and \emph{DTime} in the domains \emph{delta} and \emph{airasia} we find that $\ndsyn$ is not able to synthesize any extraction program (which is why the F1 score is "NaN"), wheras \lrsyn\ is able to synthesize programs that produce a perfect F1 score of 1.

In the domain \emph{getthere.com}, $\lrsyn$ achieves perfect extraction over all fields as compared to $\ndsyn$. This is primarily because the document formats in \emph{getthere.com} permute the constituent regions as shown in Figure~\ref{fig:formed_documents}, and \resyn\ handles such permutations naturally because it relies on landmarks and local regions, which are invariant to permutations of the regions in the document.


In the domains \emph{aeromexico} and \emph{mytrips.amexgbt} we find that both $\ndsyn$ and $\resyn$ acheive perfect F1 scores. However, this is due to some incidental aspects described below. In the \emph{aeromexico} domain, each field has  dedicated \emph{id} attributes in the DOM, such as\emph{-arrival-city-, -arrival-time, -departure-city}. Both $\ndsyn$ and $\lrsyn$ are able to latch on this attribute for extraction. These attributes remain the same in both our contemporary and longitudinal datasets, and they perform the role of landmarks, even for $\ndsyn$. Also, even the initial fine-grained whole-document blueprints in this domain exhibit no change across the contemporary and longitudinal datasets, indicating that the formats have not varied across time in this domain.
In the \emph{mytrips.amexgbt} domain, there are variations in fine-grained whole document blueprints across the two datasets which suggest that $\lrsyn$ should perform better than $\ndsyn$. When we look deeply into these variations, there are \emph{hotel} and \emph{cab} booking blocks getting added to these documents just like "getthere".
The $\ndsyn$ structure program which get synthesized for  \emph{departure time} is shown in the figure below:

\begin{figure}[H]
\vspace{-4ex}
\small
\begin{alltt}
TBODY > :nth-child(1):nth-last-child(1)
> :nth-child(2) > DIV.right_section:nth-child(1)
:nth-last-child(1) > :nth-child(10):nth-last-child(9)
\end{alltt}
\vspace{-4ex}
\end{figure}
This program iterates over the various blocks of a table, and for each block it tries to extract a region which is the $10^{th}$ child from the start and $9^{th}$ child from the end. And it so turns out that in our dataset, the \emph{hotel} or \emph{cab} blocks always have fewer than 5 lines and never pass this predicate. But, this program will break if more lines get added to these blocks, so $\ndsyn$ gets "lucky" in these cases. In comparison, the program synthesized by $\lrsyn$ zooms into the region with "Departing" as a landmark and synthesizes a simpler extraction program, which is robust to such changes in the format. It so happens that such format changes are not present in our test set.

\begin{table*}
\scriptsize
\begin{tabular}{|l|c|c|c||c|c|}
\hline
 & & \multicolumn{2}{|c||}{ Contemporary} &  \multicolumn{2}{|c|}{Longitudinal} \\
 {Fields} & Domain & $\ndsyn$ & $\resyn$ & $\ndsyn$ & $\resyn$ \\
\hline
\hline
 AIata & \multirow[b]{4}{*}{ifly}   & 0.81 & \textbf{1.00} & 0.64 & \textbf{1.00} \\
 ATime &                            & 0.76 & \textbf{1.00} & 0.62 & \textbf{1.00} \\
 DIata &                            & 0.73 & \textbf{1.00} & 0.55 & \textbf{1.00} \\
 DDate &                            & 1.00 &         1.00  & 1.00 &         1.00  \\
 DTime &  alaska                    & 0.73 & \textbf{1.00} & 0.55 & \textbf{1.00} \\
 FNum  & \multirow[t]{4}{*}{air}    & 1.00 &         1.00  & 1.00 &         1.00  \\
 Name  &                            & 1.00 &         1.00  & 0.99 &         0.99  \\
 Pvdr  &                            & --   &         --    & --   &         --    \\
 RId   &                            & 1.00 &         1.00  & 1.00 &         1.00  \\

\hline
 AIata & \multirow{9}{*}{airasia} & 0.67 & \textbf{1.00} & 0.67 & \textbf{1.00} \\
 ATime &                          & NaN  & \textbf{1.00} & NaN  & \textbf{1.00} \\
 DIata &                          & 0.67 & \textbf{1.00} & 0.67 & \textbf{1.00} \\
 DDate &                          & 0.67 & \textbf{1.00} & 0.67 & \textbf{1.00} \\
 DTime &                          & NaN  & \textbf{1.00} & NaN  & \textbf{1.00} \\
 FNum  &                          & 1.00 &          1.00 & 0.96 & 0.96          \\
 Name  &                          & 1.00 &          1.00 & NaN  & \textbf{1.00} \\
 Pvdr  &                          & 1.00 &          1.00 & 0.96 & 0.96          \\
 RId   &                          & 1.00 &          1.00 & 1.00 & 1.00          \\

\hline 
\end{tabular}
%
\begin{tabular}{|c|c|c||c|c|}
\hline
 & \multicolumn{2}{|c||}{ Contemporary} &  \multicolumn{2}{|c|}{Longitudinal} \\
 {Domain} & $\ndsyn$ & $\resyn$ & $\ndsyn$ & $\resyn$ \\
\hline
\hline\multirow{9}{*}{getthere}

 & 0.75 & \textbf{1.00} & 0.74 & \textbf{1.00} \\
 & 0.94 & \textbf{1.00} & 0.91 & \textbf{1.00} \\
 & 0.94 & \textbf{1.00} & 0.95 & \textbf{1.00} \\
 & 0.98 & \textbf{1.00} & 0.95 & \textbf{1.00} \\
 & 0.76 & \textbf{1.00} & 0.78 & \textbf{1.00} \\
 & 0.98 & \textbf{1.00} & 0.98 & \textbf{1.00} \\
 & 1.00 & 1.00 & 0.89 & \textbf{1.00} \\
 & 0.98 & \textbf{1.00} & 0.97 & \textbf{1.00} \\
 & 0.93 & \textbf{1.00} & 0.94 & \textbf{1.00} \\

\hline\multirow{9}{*}{delta}
 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & 0.94 & \textbf{1.00} & 0.95 & \textbf{1.00} \\
 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & 0.85 & \textbf{0.97} & 0.91 & \textbf{0.97} \\
 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & 1.00 & 1.00 & 1.00 & 1.00 \\

\hline 
\end{tabular}
%
\begin{tabular}{|c|c|c||c|c|}
\hline
 & \multicolumn{2}{|c||}{ Contemporary} &  \multicolumn{2}{|c|}{Longitudinal} \\
 {Domain} & $\ndsyn$ & $\resyn$ & $\ndsyn$ & $\resyn$ \\
\hline
\hline\multirow[b]{4}{*}{aero} & 1.00 & 1.00 & 1.00 & 1.00 \\
                               & 1.00 & 1.00 & 1.00 & 1.00 \\
                               & 1.00 & 1.00 & 1.00 & 1.00 \\
                               & 1.00 & 1.00 & 1.00 & 1.00 \\
\multirow[t]{4}{*}{mexico}     & 1.00 & 1.00 & 1.00 & 1.00 \\
                               & 1.00 & 1.00 & 1.00 & 1.00 \\
                               & 1.00 & 1.00 & 1.00 & 1.00 \\
                               & 1.00 & 1.00 & 1.00 & 1.00 \\
                               & 1.00 & 1.00 & 1.00 & 1.00 \\

% \hline\multirow{9}{*}{mytrips.amexgbt}
\hline
\multirow[b]{4}{*}{mytrips} & 1.00 & 1.00 & 1.00 & 1.00 \\
                            & 1.00 & 1.00 & 1.00 & 1.00 \\
                            & 1.00 & 1.00 & 1.00 & 1.00 \\
                            & 1.00 & 1.00 & 1.00 & 1.00 \\
 amex                          & 1.00 & 1.00 & 1.00 & 1.00 \\
 \multirow[t]{3}{*}{gbt}   & 1.00 & 1.00 & 1.00 & 1.00 \\
                            & 1.00 & 1.00 & 1.00 & 1.00 \\
                            & 1.00 & 1.00 & 1.00 & 1.00 \\
                            & 1.00 & 1.00 & 1.00 & 1.00 \\

\hline 
\end{tabular}
\caption{M2H F1 score details. The Pvdr field is not relevant for iflyalaskaair}
\label{tab:m2hexpmt1}
\vspace{-5ex}
\end{table*}

% sp: Move to supplement
\begin{comment}
\begin{table*}
\small
\begin{tabular}{|l|}
\hline
ifly.alaskaair.com : ArrivalAirportIata \\
\\
$\ndsyn$: \\
$L_{ex}$: $TR:nth-child(1):nth-last-child(1) > [style*="width:48\%"]:nth-child(3) >  TABLE[cellpadding="0"]$ 
\\
$[cellspacing="0"][border=0][style*="width:100\%"]:nth-child(1):nth-last-child(1) >$
\\
$TBODY:nth-child(1):nth-last-child(1) > :nth-child(1)$\\
$Text Program$ : $Extract(str, RegexPair("", "Alphanumeric"), RegexPair("Alphanumeric", "\epsilon"), -1)$\\
\smallskip\\
$\resyn$:\\
$Landmark$ : $Arrives$~,~$L_{rg}$: $\langle \mathsf{parenthops}: 0, \mathsf{siblinghops}$: $1$, $\mathsf{blueprint}$ : /TR/TD  $\rangle$\\
$L_{ex}$: $TR:nth-child(1)$ \\
$Text Program$ : $Extract(str, RegexPair("\epsilon", "Alphanumeric"), RegexPair("Alphanumeric", "\epsilon")$, \\
\hline
\end{tabular}
\caption{Synthesized extraction programs}
\label{tab:m2hprograms}
\end{table*}
\end{comment}

% sp: commenting this out for now, one example should suffice
\begin{comment}
getthere.com:Provider \\
\\
$\ndsyn$: \\
$L_{ex}$: $DIV:nth-last-child(13) > TABLE > TBODY:nth-child(1):nth-last-child(1) > :nth-child(1) > :nth-child(2)$ \\
$Text Program$ : $Extract(str, RegexPair(\epsilon, "Alphanumeric"), RegexPair(\epsilon, "WhiteSpaceNumber"), 1)$\\
\\ 
$\resyn$:\\
$Landmark$ : $Flight/Equip$\\
 $L_{rg}:\langle \mathsf{parenthops}: 0, \mathsf{siblinghops}: 1, \mathsf{blueprint}:/TD  \rangle$\\
$L_{ex}:nth-child(2)$ \\
$Text Program : Extract(str, RegexPair(\epsilon, "Alphanumeric"), RegexPair($\epsilon$, "WhiteSpaceNumber"), 1)$\\

\hline
\end{comment}



\paragraph{Synthesized programs}
Figures~\ref{lst:ndsynprogram}~and~\ref{lst:lrsynprogram} show an example extraction program synthesized by $\ndsyn$ and $\lrsyn$ respectively. More examples can be found in the supplementary material.
As seen from these, extraction programs synthesized by $\ndsyn$ programs are way more complex as they process the entire HTML page, when compared to the programs synthesized by $\lrsyn$, which only process the local region of interest.
Consequently, if the formats change, the programs synthesized by $\lrsyn$ continue to function correctly.
%
Further, the shape and size of the $\lrsyn$ programs makes them easy to 
examine by hand and gain confidence in their correctness.
\arsays{Do we have any numbers here?}
\highlightbox{
The $\lrsyn$ programs are significantly smaller compared to $\ndsyn$ programs.
%
For the web extraction component, $\lrsyn$ programs have $XXX$ components
in their CSS selectors as compared to $YYY$ for $\ndsyn$.
}


% commenting this out
\begin{comment}
\begin{table}
\small
\label{table:m2hnumberofprograms}
\begin{tabular}{|l|c|c|}
\hline
Field & \#$\ndsyn$ & \#$\lrsyn$\\
AIata & 3 & 1 \\
ATime & 2 & 1 \\
DIata & 3 & 1 \\
DDate & 3 & 1 \\
DTime & 2 & 1 \\
FNum & 1 & 1 \\
Name & 1 & 1 \\
Pvdr & 1 & 1 \\
RId & 1 & 1 \\
\hline
\end{tabular}
\caption{Getthere.com: Number of $\ndsyn$ and $\lrsyn$ programs}
\label{tab:m2h-numprograms}
\end{table}
\end{comment}

\paragraph{Number of programs} Since \resyn\ merges clusters based on ROIs rather than entire documents, this results in fewer programs synthesized by \resyn, when compared to \ndsyn.
%
For "getthere", $\lrsyn$ synthesizes only a single program for all fields: \emph{:nth-child(2)}. \ndsyn ,on the other hand, synthesizes $3$ programs each for \emph{AIata}, \emph{DIata}, \emph{DDate}, $2$ programs each for \emph{ATime} and \emph{DTime} and $1$ program for the remaining $4$ fields. 
%Table~\ref{tab:m2h-numprograms} substantiates this for fields in "getthere.com". 
We see this trend in all other domains as well, confirming our initial hypothesis that
local structure of regions of interest tend to vary less than global document
structure.

\highlightbox{
Get numbers from Anirudh}

\begin{table}
\scriptsize
\centering
\begin{tabular}{|l|c|}
\hline
Domain & Test \\
\hline
AccountInvoice & 157\\ \hline
CashInvoice & 40 \\ \hline
CreditNote & 30 \\ \hline
%New Vehicle Invoice & 34 \\ \hline
SalesInvoice & 401 \\ \hline
SelfBilledCreditNote & 146 \\ \hline
\end{tabular}
\quad
\begin{tabular}{|l|c|}
\hline
Domain & Test \\
\hline
aeromexico & 303\\ \hline
getthere & 155 \\ \hline
westjet & 500 \\ \hline
amex & 619 \\ \hline
\end{tabular}
\caption{Test set sizes for Finance and M2H-Images datasets. Train set size is $10$ for all the domains}
\label{tab:imagesdata}
\end{table}



\begin{table}
\scriptsize
\begin{tabular}{|c|l|c|c|c|}
\hline
{Domain} & Fields & $\afr$ & $\resyn$\\
\hline\multirow{9}{*}{AccountsInvoice}
  & Amount & 0.99 & \textbf{1.00} \\
  & Chassis & 0.82 & \textbf{0.99} \\
  & CustAddr & 0.98 & \emph{0.96} \\
  & Date & 0.93 & \textbf{0.98} \\
  & Dnum & 0.96 & \textbf{0.97} \\
  & Engine & 0.82 & \textbf{1.00} \\
  & InvoiceAddress & 0.90 & \textbf{0.95} \\
  & Model & 0.75 & \textbf{1.00} \\

\hline\multirow{8}{*}{CashInvoice}
  & Amount & 1.00 & 1.00 \\
  & Chassis & 0.99 & 0.99 \\
  & CustAddr & 0.99 & \emph{0.97} \\
  & Date & 0.99 & 0.99 \\
  & Dnum & 0.96 & 0.96 \\
  & Engine & 0.93 & \textbf{0.95} \\
  & InvoiceAddress & 0.99 & 0.99 \\
  & Model & 0.99 & \textbf{1.00} \\

\hline\multirow{5}{*}{CreditNote}
  & Amount & 1.00 & 1.00 \\
  & CreditNoteAddress & 0.99 & \textbf{1.00} \\
  & CreditNoteNo & 0.94 & \emph{0.93} \\
  & CustRefNo & 1.00 & 1.00 \\
  & Date & 1.00 & 1.00 \\
  & RefNo & 1.00 & 1.00 \\

\hline\multirow{6}{*}{SalesInvoice}
  & Amount & 1.00 & 1.00 \\
  & CustomerReferenceNo & 1.00 & 1.00 \\
  & Date & 1.00 & 1.00 \\
  & InvoiceAddress & 0.94 & \textbf{0.99} \\
  & RefNo & 0.99 & 0.99 \\
  & SalesInvoiceNo & 0.99 & 0.99 \\

\hline\multirow{6}{*}{SelfBilledCreditNote}
  & Amount & 1.00 & 1.00 \\
  & CustomerAddress & 1.00 & \emph{0.99} \\
  & CustomerReferenceNo & 0.99 & 0.99 \\
  & Date & 1.00 & 1.00 \\
  & DocumentNumber & 1.00 & 1.00 \\
  & VatRegNo & 1.00 & 1.00 \\

\hline
\end{tabular}
\caption{F1 scores for Finance dataset}
\label{tab:financedataset}
\end{table}

\begin{table}
\scriptsize
\begin{tabular}{|l|p{1.5cm}|c|c|}
\hline
Fields & {Domain} & $\afr$ & $\resyn$\\
 \hline
AIata & \multirow{9}{*}{aeromexico}        & 0.62 & \textbf{0.65} \\
ATime &                                 & 0.69 & \textbf{0.99} \\
DIata &                                 & 0.36 & \textbf{0.66} \\
DDate &                                 & 0.71 & \textbf{0.89} \\
DTime &                                 & 0.65 & \textbf{0.97} \\
FNum  &                                 & 0.66 & \textbf{0.83}  \\
Name  &                                 & 0.96 & \textbf{0.98}  \\
Pvdr  &                                 & 0.69 & \textbf{0.78}  \\
RId   &                                 & 1.00 & 1.00            \\
 
\hline
\end{tabular}
%
\begin{tabular}{|p{1.5cm}|c|c|}
\hline
{Domain} & $\afr$ & $\resyn$\\
\hline
\multirow{9}{*}{getthere}  & 0.94 & \textbf{1.00} \\
                           & 0.87 & \textbf{1.00} \\
                           & 0.93 & \textbf{1.00} \\
                           & 0.96 & \textbf{0.99} \\
                           & 0.88 & \textbf{1.00} \\
                           & 0.94 & \textbf{1.00} \\
                           & 0.99 &         0.99  \\
                           & 0.75 & \textbf{1.00} \\
                           & 0.89 & \textbf{0.95} \\
 
\hline
\end{tabular}
%

\begin{tabular}{|l|p{1.5cm}|c|c|}
\hline
{Fields} & Domain & $\afr$ & $\resyn$\\
\hline
AIata & \multirow[b]{4}{*}{itinerary.}     & 0.94 & \textbf{0.99} \\
ATime &                                    & 0.90 &   \emph{0.88} \\
DIata &                                    & 0.93 & \textbf{0.98} \\
DDate &                                    & 0.93 & \textbf{1.00} \\
DTime &  \multirow[t]{4}{*}{westjet}       & 0.94 & \textbf{0.95} \\
FNum  &                                    & 0.96 & \textbf{1.00} \\
Name  &                                    & 0.60 & \textbf{0.61} \\
Pvdr  &                                    & 0.95 & \textbf{1.00} \\
RId   &                                    & 1.00 &         1.00 \\
 
\hline
\end{tabular}
%
\begin{tabular}{|p{1.5cm}|c|c|}
\hline
{Domain} & $\afr$ & $\resyn$\\
 \hline
\multirow[b]{4}{*}{mytrips}  & 0.85 & \textbf{0.98} \\
                             & 0.97 & \textbf{1.00} \\
                             & 0.96 & \textbf{0.99} \\
                             & 0.93 & \textbf{1.00} \\
\multirow[t]{4}{*}{amexgbt}  & 0.99 & \textbf{1.00} \\
                             & 0.98 & \textbf{1.00} \\
                             & 0.98 & \textbf{1.00} \\
                             & 0.91 & \textbf{0.99} \\
                             & 0.61 & \textbf{0.96} \\

\hline
\end{tabular}
\caption{F1 Score for Images M2H Dataset}
\label{tab:m2himages}
\vspace{-5ex}
\end{table}


\begin{comment} 
\hline\multirow{9}{*}{ifly.alaskaair}   
 & AIata & 0.98 & \textbf{1.00} \\
 & ATime & 0.95 & \textbf{0.99} \\
 & DIata & 0.98 & \textbf{1.00} \\
 & DDate & 0.98 & \emph{NaN} \\
 & DTime & 0.95 & \textbf{0.98} \\
 & FNum & 0.97 & \textbf{1.00} \\
 & Name & 0.98 & 0.98 \\
 & Pvdr & 0.93 & \textbf{0.99} \\
 & RId & 1.00 & \emph{0.86} \\
\end{comment}

% move to supplement
\begin{comment}
\begin{table*}
\small
\begin{tabular}{|l|l|l|}
\hline
{Domain} & Manually provided landmarks & Learnt landmarks \\
\hline
ifly.alaskaair & 
     Departs, Arrives, Term/Gate,  & Departs, Arrives, \textbf{Confirmation code: >> Term/Gate,}  \\
   & Travellers, Confirmation code &  Travellers, \textbf{Travelers: >> Confirmation code}  \\
\hline
\end{tabular}
\caption{Landmarks for M2H dataset}
\label{tab:m2hlandmarks}
\end{table*}
\end{comment}

\paragraph{Quality of Inferred Landmarks}
We infer landmarks automatically using the techniques and scoring functions mentioned in Section~\ref{sec:algorithms} and~\ref{sec:instantiations}.
%
To check the quality of landmark inference, we also asked data annotators to tag the landmarks manually.
%
\highlightbox{
In $57$ out of $63$ clusters across all fields, the inferred landmarks are exactly the same as manually provided landmarks.
%
In $5$ of the remaining $6$ cases, the human annotator agreed that the inferred landmark 
was of equal quality.
}
%
In the remaining $1$ case, the algorithm chose the human annotated landmark as well, but 
in addition chose a disambiguating hierarchical landmark of low quality.
%
In particular, it disambiguated the term \emph{Name} occurred in reference to both
the name of the passenger and the name in the  billing address.
%
Here, the algorithm chose to disambiguate using the term \emph{Meal}, i.e.,
passengers have a meal preference while the billed person does not.
%
We refer the readers to the supplementary material for the list of all landmarks inferred.
% \arsays{We need numbers here, and the example should be brought back in the right form}


\subsection{Form Image Extraction}
We consider two datasets of form images:
(1) {\em Finance} dataset: This consists of ~850 images of receipts, purchase orders, credit notes, sales invoice and similar such documents. Figure~\ref{fig:formed_documents}(c)~shows one such image of a sales invoice. The training and test data are from the same time period. Hence this dataset is used to do contemporary evaluation.
(2) {\em M2H-Images} dataset: We convert M2H emails from $4$ domains to images and extract the same fields as before. This represents common scenarios in practice where HTML documents such as booking mails or receipts may be printed and then scanned again for data extraction where the original structure is lost. Table~\ref{tab:imagesdata} shows the test data sizes for each domain in both these datasets. We use a training data size of $10$ in all our image extraction experiments. In M2H dataset, the test data contains emails from a different time period than the ones in the training set. Hence this dataset is used to do a longitudinal evaluation.
\arsays{Somebody will definitely ask why not all 6 domains}


We first pre-process these images to make them sharper and perform optical character recognition (OCR) on them. This provides us with bounding boxes and text for these images, and we operate on top of this input. For our experiments, we use the OCR offering from Microsoft Azure~\cite{AzureOCR}. We compare $\lrsyn$ with a custom neural model fine-tuned using Azure Form Recognize (\afr)~\cite{AFR}, which is a cloud-based Azure Applied AI Service. We use a sample of $10$ documents as training data for each domain in our experiments. We do not handle issues like spelling errors in OCR output in the current work and employ heuristics to correct them.

\paragraph{Overall Results}
Table~\ref{tab:imagesoverall}~shows the average precision, recall, F1 and accuracy scores for \afr\ and \ndsyn\, for both the Finance and M2H-image datasets. The scores are weighted by the test sizes across various extraction tasks. Unlike $\afr$ which is a neural model, $\lrsyn$ synthesizes programs on top of OCR boxes. As we can see from the table, $\lrsyn$ performs marginally better than $\afr$ on the Finance dataset. This is mainly because the test data does not have variations when compared to training set.  $\lrsyn$ outperforms $\afr$ in the M2H-Images dataset with a F1 score of $0.95$ as compared to $0.87$, since the test data in this dataset contains images from a different time period, and these images have many variations when compared to the training set.
%
\highlightbox{
$\lrsyn$ outperforms a state-of-the-art industrial form extraction system trained on
\arsays{$10^x$s} of images, with just $10$ training images per field, having a precision
of $0.95$ vs $0.87$ on the M2H-Image dataset.
}

\begin{table}
\scriptsize
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|l|c|c|c|}
\hline
Metric & $\afr $ & $\lrsyn$\\
\hline
Avg. Pre.  & 0.98	& 0.99 \\ \hline
Avg. Rec.  & 0.96	& 0.99 \\ \hline
Avg. F1  & 0.97	& 0.99 \\ \hline
\end{tabular}
\caption*{Finance dataset}
}
\hfill
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|l|c|c|c|}
\hline
Metric & $\afr $ & $\lrsyn$\\
\hline
Avg. Prec.  & 0.85	& 0.95 \\ \hline
Avg. Rec.  & 0.91	& 0.95 \\ \hline
Avg. F1  & 0.87	& 0.95 \\ \hline
\end{tabular}
\caption*{M2H-Images dataset}
}
\vspace{-3ex}
\caption{Average precision, recall, F1 numbers on Finance and M2H-Images dataset}
\label{tab:imagesoverall}
\vspace{-3ex}
\end{table}

\paragraph{Detailed comparison}
Table~\ref{tab:financedataset}~shows the results of $\afr$ and $\lrsyn$ on the Finance dataset with respect to $34$ extraction tasks. $\lrsyn$ performs better than $\ndsyn$ in $12$ out of the $34$ cases and is on par on the rest, with significant gains in some domains like "AccountsInvoice". 

Even though the neural model in $\afr$ is trained with thousands of invoices and receipts, and further fine-tuned with our training data, we observe that it is sensitive to the region coordinates in a given document. If these regions translate slightly or if the document scan is tilted, $\afr$ extraction is erroneous. $\lrsyn$ is partially robust to such changes as the region programs start from a landmark value, and is agnostic to changes happening in the other regions. 

Also, as we can note from the table, $\afr$ is marginally better than $\lrsyn$ in some of the extraction tasks. This can be attributed to the absence of the boundary pattern in some of the test documents resulting in incorrect extractions. $\afr$, on the other hand, in all likelihood, understands concepts like "address" and can extract irrespective of the presence of a boundary pattern. $\lrsyn$ can be improved further by incorporating such a semantic layer in its processing. 

Table~\ref{tab:m2himages}~shows the results of $\afr$ and $\lrsyn$ on the M2H dataset with respect to $45$ extraction tasks. This dataset exhibits more variations at the visual level as compared to the Finance dataset. $\lrsyn$ performs better than $\ndsyn$ in $35$ out of the $45$ tasks and is on par on most of the remaining extraction tasks. This is mainly because $\lrsyn$ first locates the region of interests and then extracts values from these regions. 

\paragraph{Synthesized programs}
Here is an example region and text program synthesized for the "Date" field in \emph{SalesInvoice} document, with respect to a landmark "Date". \\
Region program: $Extend("Date", Relative(Right, EOL, false)$ \\
Text program: Extract a substring between ":" and EOL\\

%\begin{lstlisting}[caption = \lrsyn\ region program for Date, captionpos = b, basicstyle=\small, frame = single, label = lrsynprogram_date ]
%Region program: Extend("Date", 
%                Relative(Right, EOL, false)
%Text program: Extract a substring 
%between ":" and EOL
%\end{lstlisting}
The region program starts from the landmark "Date" and extends right to collect all boxes until the end of line (EOL). And the corresponding text program extracts the text between a colon and EOL. We refer the readers to Table~\ref{}~ in the Appendix for more examples. \spsays{looks ugly, needs more work!!}

\paragraph{Summary of results}
In the HTML domain, the prior work \ndsyn\ is a high-performing system with F1 scores in the range of 0.9. \lrsyn\ is able to push the F1 scores to a perfect 1.0 in most cases. In longitudinal scenarios, \lrsyn\ improves \ndsyn\ in 24 out of 53 fields, with significant lift in F1 scores in many cases.
In the images domain, even with very little training data, \lrsyn\ matches AFR, which is a released product on contemporary settings, and outperforms AFR in longitudinal settings. In addition, \lrsyn\ produces simpler interpretable programs that match human intuition for extraction, and are much easier to maintain. Hence, we see a lot of promise in this approach.

%As seen from the table, extraction programs synthesized by $\lrsyn$ are simple. The first program starts at the landmark and collects all the boxes to its right until it hits an EOL. Likewise, the Chassis program starts with the landmark, comes one step down and extends to the right till it hits a pattern.


% sp: moving this to the supplementary material
\begin{comment}
\begin{table*}
\small
\begin{tabular}{|l|}
\hline
Sale Invoice : Date \\
Landmark: "Date:" \\
Region program: Extend("Date", Relative(Right, EOL, false) \\
Text program: Extract a substring between ":" and EOL \\
\hline 
Accounts Invoice: Chassis Number \\
Landmark: "Chassis Number" \\
Region program: Extend(Extend(input, Absolute(down, 1)), Relative(Right, DATE, false)) \\
Text Program: Take all the strings in this path \\
\hline
Accounts Invoice : InvoiceAddress \\
Region program: ExtendLineItems("Invoice Name \& Address", Relative(down, "Model SKU")) \\
Text Program: Take all the strings in this path \\
\hline
\end{tabular}
\caption{Synthesized extraction programs \spsays{Improve presentation}}
\label{tab:imageprograms}
\end{table*}
\end{comment}

\paragraph{Efficiency of Data Extraction}
%
Formed document data extraction programs are sometimes run on extremely large
datasets, and hence, their efficiency becomes a concern.
%
For example, an industrial system that was the source of the M2H data processes
over $3 \times 10^8$ emails each day.
%
\highlightbox{
  The $\lrsyn$ programs for the M2H dataset outperform their $\ndsyn$
  counterparts by \arsays{AAAX}, with an average processing time of $XXX$~ms vs. $YYY$~ms.
}
%
We believe this is mainly due to the extremely cheap landmark location step,
with the more expensive parts of the program only running on the small ROI.

==> resyn.tex <==
\begin{comment}
Our approach to Hierarchical Synthesis is based on narrowing down the regions in an hierarchical fashion using \textbf{Landmarks} and synthesizing extraction program(s) for the final region. Our hypothesis is that it is easier to narrow down on the regions in a sequence of individually robust steps using landmarks rather than all at once.
\end{comment}

\spsays{Algorithms need few more iterations. Did a single pass on Algorithms 1, 2 and 3 }

\spsays{We represent clusters as a tuple (D, L, M) consisting of documents, landmark, region-growing metadata}


\begin{algorithm}
\small
\caption{Region Synthesis Algorithm (Given a cluster of documents)}
\label{algo:landmarks1}
\begin{algorithmic}[1]
\Require Annotated documents $D$ from a cluster $C$
\Require Field $F$
\State $\mathsf{landmarks} \gets LearnLandmarks(D, F)$
\State $\PP \gets \mathsf{Learn}(D_c, \mathsf{landmarks}[1], F, \LL)$
\State \Return $\PP$
\State
\Function{LearnLandmarks}{$D, F$}
\State $cand \gets \mathsf{GetCandidates}(D,F)$
\ForEach {$candidate \; c_i \in cand$}
\State $\{c_i,S_i\} = \mathsf{ScoringFunction}(D, c_i, F)$
\EndFor
\State \Return top k landmark candidates $L$ by score
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\small
\caption{LearnHierarchyOfLandmarks}
\label{algo:hierarchy}
\begin{algorithmic}[1]
\Require Annotated documents $D$ from a cluster $C$
\Require Field $F$
\State $\mathsf{landmarks} \gets \langle\rangle$
\State $\mathsf{noisy} \gets False$
\Do
\State $\mathsf{landmark} \gets LearnLandmarks(D, F)$
\State $\mathsf{landmarks} \gets \mathsf{landmarks} + \mathsf{landmark}$
\State occurrences = GetOccurrences(D, landmark)
\If {$occurrences == 1$}
\State break
\EndIf
\State bp = GetBluePrint(GrowRegion(D, landmark, F))
\ForEach {$document \; d \in D$}
\ForEach {$occurrence \; o \in occurrences$ (excluding the selected landmark)}
\State $\mathsf{region} \gets \mathsf{GrowRegion}(d, o, F)$
\If {$bp == GetBluePrint(region)$}
    \State $\mathsf{noisy} \gets True$
    \State break
\EndIf
\EndFor
\EndFor
\State $\mathsf{F} \gets landmark$
\doWhile {$noisy \; == \; True$}
\State \Return landmarks
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\small
\caption{ClusterAndLearnLandmarks (Needs more work)}
\label{algo:cluster}
\begin{algorithmic}[1]
\Require Annotated documents $D$
\Require Field $F$
\State $\mathsf{clusters} \gets \mathsf{L0Clustering}(D,\mathsf{GetBluePrints}(D))$
\State $\mathsf{C} \gets$ Merge clusters with size < $k$, order by size
\State $\mathsf{BaseClusters} \gets C[1]$
\State $\mathsf{i} \gets 2$
\While {$i \leq \mathbf{card}(B)$}
    \State $\mathsf{merged} \gets False$
    \ForEach {$\mathsf{basecluster} \; cluster \in BaseClusters$}
    \State ret = $\mathsf{Merge}(C[i], cluster, F)$
    \If{$ ret $}
    \State $\mathsf{merged} \gets True$
    \State $\mathsf{break}$
    \EndIf
    \EndFor
    \If{$ not \; ret $}
    \State  $\mathsf{BaseClusters} \gets \mathsf{BaseClusters} \; + \; C[i]$
    \EndIf
\EndWhile
\State \Return $BaseClusters$
\State
\Function{Merge}{$\mathsf{cluster} \; C, cluster \; \mathsf{baseCluster}$}
    \State $\mathsf{L} \gets \mathsf{Landmark(baseCluster)}$
    \State $\mathsf{regions} \gets \langle \rangle$ 
    \ForEach {$\mathsf{d_i} \; \in cluster$}
    \State $\mathsf{regions} \gets \mathsf{regions} + \mathsf{GrowRegion(d_i, L, F)}$
    \EndFor    
    \State $\mathsf{regionHash} \gets \mathsf{GetBluePrint}(regions)$ 
    \If{$regionHash = \mathsf{GetBluePrint}(baseCluster)$}
    \State \Return $True$
    \EndIf
    \State \Return $False$
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\small
\caption{Prediction}
\label{algo:predict}
\begin{algorithmic}[1]
\Require Document $D$
\end{algorithmic}
\end{algorithm}

\section{HTML extraction and $\resyn$}


\section{Structured image extraction and $\resyn$}

\begin{comment}
\begin{algorithm}
\small
\caption{Landmark Detection}
\label{lst:cover}
% \hspace{-4.5in}
\flushleft $\mathsf{Landmark Detection}(D,O_R,F)$
\begin{algorithmic}[1]
\Require Documents $D = \{D_1,D_2,...,D_n\}$
\Require Output Regions $O_R = \{O_1,O_2,O_3,...,O_n\}$ for $D_i$
\Require Field $F$
\State $L_c=\phi$ where $L_c$ is set of Lmk candidate 
\State \textbf{for each}$D_i \in D$ \textbf{do}
\State \hspace{\algorithmicindent} \textbf{if }$L_c = \phi$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$L_c \gets FindNGrams(D_i)$
\State \hspace{\algorithmicindent}\textbf{else}
\State\hspace{\algorithmicindent}\hspace{\algorithmicindent}$L_c \gets L_c \cap FindNGrams(D_i)$
\State \textbf{for each} $D_i \in D$ \textbf{do}
\State \hspace{\algorithmicindent}\textbf{for each} $L_i \in L_c$ \textbf{do}
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}$l_r \gets ComputeSmallestRegion(Ls,D)$
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}$R_{L_i} \gets RegionGrwoingLearn(L_i,O_R,F)$
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}$R_{hash} \gets ComputeBlueprint(R_i)$ for each $R_i \in R_{L_i}$ 
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}Steps $S \gets Max(ComputeSteps(R_i)$ for each $R_i \in R_{L_i}$ 
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}Find $l_{r'} = l_r \notin R_{L_i}$ 
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}$R'\gets RegionGrowingPredict(L_i,S,D)$
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}$R_{hash}' \gets ComputeBlueprint(R_i')$ for each $R_i' \in R_{L_i}' $
%New logic added
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}$R_{noisy} =R_{hash}' \in R_{hash} $
\State  \hspace{\algorithmicindent}\hspace{\algorithmicindent}Store $R_{hash}' \notin R_{hash}$ 
%s_n,s_r,s_v are scores for noisy, region, and visual 
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$s_{noisy}=1/(|R_{noisy}|+1)$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$s_{region}=1/(Argmax(Width(R_{L_i})))$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$D_{visual} = ComputeVisualDistance(l_i,o_i)$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$s_{visual}= 1/ArgMax(D_visual)$
\State Compute Average across each score for $l_i$ to find ${S_{n_{l_i}},S_{r_{l_i}},S_{v_{l_i}}}$
\State Previous Noisy Score $S_{N_prev} = 0$ 
%Run till noisy score is not 1
\State \textbf{do}
%TODO: Add-tie breaker conditions  
\State \hspace{\algorithmicindent} $L_s \gets \{ l_i | Argmax(ComputeScore(S_{r_{l_i}},S_{v_{l_i}})) \land S_{n_{l_i}} > S_{N_{prev}} \}$
\State  \hspace{\algorithmicindent} $S_{N_{prev}} = S_{n_{l_i}}$
\State \textbf{while $S_{n_{l_i}}!=1$}
\State \Return $L_s$
\State
\Function{FindNGrams}{$D_i$}
 \State $N \gets GenerateNGram(D_i)$
 \State $N$
%Insert Conditions
%Ngram length > 2 
%Should not be all number 
%Shouldn't be output token 
%All ngram tokens shouldn't be stopwords or words in blacklist = {"canada", "seattle", "atlanta", "international", "airport", "qatar", "checked", "duration"} 
\State \Return $\RR$
\EndFunction
\State
\Function{ComputeVisualDistance}{$l_i,o_i$}
 \State Let $Box_{l_i} \gets\{x_{l_{left}},x_{l_{right}},y_{l_{top}},y_{l_{bottom}}\} $
 \State Let $Box{o_i} \gets\{x{o_{left}},x_{o_{right}},y_{o_{top}},y_{o_{bottom}}\} $
 \State $x_1 = (x{l_{left}}+x_{l_{right}})/2$
 \State $x_2 = (x{o_{left}}+x_{o_{right}})/2$
 \State $y_1 = (y{l_{top}}+y_{l_{bottom}})/2$
 \State $y_2 = (y{o_{top}}+y_{o_{bottom}})/2$
 \State $D=\sqrt{(x_{1}-x_{2})^2+(y_{1}-y_{2})^2}$ 
\State \Return $D$
\EndFunction
\State
\Function{ComputeScore}{$S_{r},S_{v}$}
 \State $S =\log_{10}(S_{r})+\log_{10}(S{v})$  
\State \Return $S$
\EndFunction

\end{algorithmic} 
\end{algorithm}

\begin{algorithm}
\small
\caption{Clustering And Landmark Detection}
\label{lst:cover}
% \hspace{-4.5in}
\flushleft $\mathsf{ClusteringAndLmkDetection}(D,T,K,F)$
\begin{algorithmic}[1]
\Require Documents $D = \{D_1,D_2,...,D_n\}$
\Require Threshold for big clusters $T$
\Require Number of Lmk Candidates $K$
\Require Field $F$
\State \textbf{for each} $D_i \in D$ \textbf{do}
\State \hspace{\algorithmicindent} $F \gets ComputeBlueprint(D)$
\State Let Big Clusters $B = \{B_1,B_2,...,B_n\}$ 
%L0 clustering find better name for L_0
\State $L_0 \gets$ Merge Based on Blueprint F
\State Let $L_0=\{\{D_1,D_x,...\},\{D_3,D_y,..\},\{D_n,D_z,...\}\}$
%L1 clustering
\State \textbf{for each} $C_i \in L_0$ \textbf{do}
\State \hspace{\algorithmicindent}\textbf{if} $|C_i| \ge T$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$B_i \gets C_i$
\State \hspace{\algorithmicindent}\textbf{else}
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$S_i \gets C_i$

\State \textbf{if} $|B_i|=0$
\State \hspace{\algorithmicindent}$B_1 \gets C_i \forall C_i \in L_0$
\State \hspace{\algorithmicindent}$S_i \gets \phi$
\State \textbf{for each} $B_i \in B$ \textbf{do}
%find O for each document in B_i
\State \hspace{\algorithmicindent} $L \gets LandmarkDetection(B_i,O,F)$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\textbf{for each} $l_i \in L$ \textbf{do}
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}$R_{B_{l_i}}\gets RegionGrowingLearn(l_i,O,F)$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}$H_{B_{l_i}}\gets ComputeBlueprint(R_{B_{l_i}})$ where $H = ROIHash$ 
\State $H_{score}=\{(H_B_{l_1},0),(H_B_{l_2},0),...,(H_B_{l_i},0)\}$ where $H_B_{l_i} \in H_{B_{l}}$ 
\State $C=\{B_1\}$ where $B1=Biggest Cluster$
%Sort P on Cluster Size
\State $P = (B-\{B_1\}) \cup S$
\State \textbf{for each} $P_i \in P$ \textbf{do}
\State \hspace{\algorithmicindent} \textbf{for each} $C_j \in C$ \textbf{do}
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$L' = L_{B}$ where $B = Argmax(|B| \in C)$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$R_{p_i} \gets RegionGrowingLearn(L_{k}',O_{p_{i}},F) \forall L_{k}' \in L'$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}$H_{p_i}' \gets ComputeBlueprint(R_{p_k})\forall R_{p_k} \in R_{p_i}$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\textbf{if} $H_{p_i}' \cap H_{C_j} \to$ \o
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}$C \gets P_i$; Add $P_i$ to $C$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\textbf{else}
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\textbf{for each}$H_x \in H_{p_i}$' \cap H_{C_j}$ \textbf{do}
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}H_{score}[H_x] =H_{score}[H_x]+1$
\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}$C_j \gets C_j \cup P_i$

\State \Return C
\end{algorithmic} 
\end{algorithm}
\end{comment}

\begin{comment}
\begin{example}
  One possible approach to achieve the extraction of departure times is in
  $3$ steps:
  %
  \begin{inparaenum}[(a)]
    \item First, extract the itinerary table from the email,
    \item Second, from the itinerary table extract the row corresponding to
      each flight; and
    \item Finally, extract the cell corresponding to the departure time from
      the row.
  \end{inparaenum}
  %
  There are several advantages of doing this extraction in steps.
  %
  In Figure~\ref{fig:roi}, we illustrate one hierarchy of regions of interest
  that would be produced during this extraction.

  During a one shot extraction, an extractor needs to consider multiple
  issues at once:
  %
  \emph{
  Which of the tables in the email are itinerary tables?
  %
  Which of the rows in the itinerary tables correspond to flights and which
  correspond to advertisements?
  %
  In the rows, which cell contains the departure time?
  }
  %
  In practice, a program synthesizer or ML model handling all these issues at
  once is more likely to produce incorrect output both due to the inherent
  complexity of the problem and due to the technique 
  %
  On the other hand, separating concerns, we can narrow down these regions progressively and synthesizer has to take into account only the final region to synthesize an extraction program. This results in simpler programs as well.
  %
  \qed
\end{example}

%
Further, by proceeding one step at a time, it is possible to use different
extractors in different steps. In this work, we follow simple traversal techniques to narrow down the regions, but one can imagine employing ML models for narrowing down the regions.
\end{comment}
\begin{comment}
It is frequently the case that different extractors are suited for different
steps.
%
For example, ML models are often more suited to the task of narrowing down
from a whole document to a smaller region that contains all the output
regions, while programs produced by a program synthesizer are more adept at
extracting the intended output from the smaller region.
\end{comment}
%

\begin{comment}
A \emph{sequence extractor} $\SeqExtractor$ is given by a sequence of
extractors $\Extractor_0 \cdot \ldots \cdot \Extractor_k$.
%
The sequence of extractors behave as a single extractor as follows:
%
\begin{itemize}
  \item For a sequence extractor $\SeqExtractor = \Extractor_0$ consisting of
    a single extractor we define $\SeqExtractor(\doc) = \Extractor_0(\doc)$,
    and
  \item For a sequence extractor $\SeqExtractor = \Extractor_0 \cdot \SeqExtractor'$,
    we define $\SeqExtractor(\doc) =
    \SeqExtractor'(\region_0)\ldots\SeqExtractor'(\region_n)$ where
    $\Extractor_0(\doc) = \region_0\ldots\region_n$.
\end{itemize}
%
Note that we are generalizing the definition extractor to act both on
documents as well as regions.
%
Henceforth, we use the term extractor to also mean sequence extractor,
assuming that the intended meaning is clear from the context.

During a sequence extraction, each extraction phase produces intermediate
output regions.
%
We dub the regions at each intermediate step the \emph{regions of interest}
(ROIs) at that step.
%
\end{comment}

\begin{comment}
\section{The \technique Algorithm}
Algorithm~\ref{algo:hierarchical-extraction} depicts the high level procedure
of algorithm \technique.
%
The algorithm takes as input a set of examples $\Examples^*$ and a set of
learners $\mathsf{Learners}$.
%
First, it chooses non-deterministically whether to do a one-shot extraction
or a hierarchical extraction.
%
If a one-shot extraction is chosen, the procedure \textsc{Extract} picks a
learner from $\mathsf{Learners}$ and returns the result of that learner on
the given examples.

On the other hand, if a hierarchical extraction is chosen, for each example
$\doc \mapsto \region_0\ldots\region_n$, we first identify the regions of
interest $\region_0^*\ldots\region_m^*$ for the current step.
%
The first extraction task is to hierarchically extract the regions of
interest from each document.
%
We do this using a recursive call to \textsc{HierarchicalExtract} on examples
of the form $\doc \mapsto \region_0^*\ldots\region_m^*$ for each document.
%
Now, the second extraction task is to extract the intended outputs from the
regions of interest.
%
For each region of interest $\region^*_i$, we associate corresponding output
$\region^{i_1}\ldots\region^{i_k}$ where $\region_{i_*}$ consists of all the
output regions that are contained in the region on interest $\region^*_i$.
%
Now, the examples for the second recursive call is given by the union of such
examples over all documents.
%
The final returned extractor is the results of the individual recursive calls
in sequence.

\begin{algorithm}
\small
\caption{Hierarchical Data Extraction}
\label{algo:hierarchical-extraction}
\arsays{No one will understand the indexing notation}
\begin{algorithmic}[1]
\Require Extraction examples $\Examples^*$
\Require Learners $\mathsf{Learners} = \learner_0, \ldots, \learner_n$
%
\State \Return \Call{HierarchicalExtract}{$\Examples^*, \mathsf{Learners}$}
\State
%
\Function{HierarchicalExtract}{$\Examples, \mathsf{Learners}$}
\State Let $\Examples$ be $\{ \doc \mapsto \region_0\ldots\region_n \}_i$
\If{*} \Comment{One-shot vs. Hierarchical}
\State \Return \Call{Extract}{$\Examples, \mathsf{Learners}$}
\Else
\State $\{ \doc \mapsto \region_0^*\ldots\region_m^* \}_i \gets \Call{IdentifyROI}{\Examples}$
\State $\Examples' \gets \{ \doc \mapsto \region_0^*\ldots\region_m^*\}_i$
\State $\Examples'' \gets \Call{Flatten}{\{
    \{
        \region^* \mapsto \region_{p_0}\ldots\region_{p_k} \mid \region_{p_k} \containedin \region^*
    \}_j
\}_i}$ 
\State $\SeqExtractor_0 \gets \Call{HierarchicalExtract}{\Examples', \mathsf{Learners}}$
\State $\SeqExtractor_1 \gets \Call{HierarchicalExtract}{\Examples'', \mathsf{Learners}}$
\EndIf 
\State \Return $\SeqExtractor_0 \cdot \SeqExtractor_1$
\EndFunction
%
\State
%
\Function{Extract}{$\Examples, \mathsf{Learners}$}
\State $\learner \gets \text{Pick learner from $\mathsf{Learners}$}$
\State \Return $\learner(\Examples)$
\EndFunction
\end{algorithmic}
\end{algorithm}

\paragraph{Identifying Regions of Interest}

\begin{itemize}
  \item Landmarks using delimiters
  \item Unsupervised clustering + limited DSL for predicates
  \item Common segments across multiple inputs and input formats
\end{itemize}

\paragraph{Learner Agnostic Robustness}
%
To ensure the robustness of the full sequence extractor produced by
Algorithm~\ref{algo:hierarchical-extraction}, we ensure the robustness of the
extractor produced at each step.
%
Recall that we defined robustness using the notion of admissible inputs
$\adocs \subseteq \docs$, the set of input documents similar enough to the
example inputs, on which the sequence extractor is expected to operate
correctly.
%
However, $\adocs$ is not provided as an input to the procedure.
%
Instead, we attempt to make the extractor robust using \emph{perturbations}.

Given an example $\ex = \doc \mapsto \region_0\ldots\region_n$, a
\emph{perturbation strategy} produces additional examples of the form
$\doc' \mapsto \region_0'\ldots\region_n'$ derived from $\ex$.
%
Informally, given an example, a perturbation strategy generates multiple new
examples similar to the original.
%
Our perturbation strategies make minor changes to the input $\doc$ which are
likely to change the expected output in a predictable way.

\begin{example}
    Changing formats, changing entities, adding ads in emails, etc
\end{example}

\section{Introduction}
Programs synthesized using current benchmark examples aren't robust enough, they do not give correct outputs on similar unseen inputs. So following set of techniques were used for achieving robustness.

\section{Techniques}
Each of these ideas are cover one or more following points of robustness:
\begin{itemize}
    \item Robust program is based on global property of input. For example, for TText this can be some character/string like delimiters. 
    \item The program tokens should be generic enough to cover unseen inputs. For example, TText regex token "Words/dots/hyphens" is more generic than "Alphanumeric".
\end{itemize}
 
\subsection{Perturbation}
The idea focuses on second point of robustness, where adding adding different varied input examples should guide the DSL to learning robust program. Introducing variety into constraints also help in the synthesizing program based on global property as different input representations go out of scope of DSL tokens.\\ \\
\begin{algorithm}[H]
\caption{Generate robust program: Perturbation}
\begin{algorithmic}[1]
    \Require Original benchmark constraints $C_1$, DSL Ranker $R$
    \State Generate new constraints $C_2$ using entity and character replacement in $C_1$, $C_2 = PERTURB(C_1)$\\
    \State Synthesize program $P = SYNTHESIS(C_2,R)$
                           %\tcp*{degree of robustness checked manually}
                           \Comment{degree of robustness checked manually}
    \If{$P$ is robust enough}        
    \State {End}                       
    \Else {$C_2 = PERTURB(C_2)$to break program token in $P$, Go to 3}
    \EndIf
\end{algorithmic}
\end{algorithm}

\subsection{Improved Ranking}
DSL ranking is tweaked to give preference to certain characters based on which the relevant programs will get boost. In TText, these turn out to be common delimiters as pointed out in robustness earlier. For example, Words/dots/hyphens ◦ Comma to Comma, i.e. boost programs having only Comma than xyz ◦ Comma.\\ \\
\begin{algorithm}[H]
\caption{Generate robust program: Tweaked Ranking}
    Given: original benchmark constraints $C_1$, DSL Ranker $R$ \\
    Create new ranker $R_{mod}^1$ wherein delimiter is taken from user input.\\
    Synthesize robust program $P = SYNTHESIS(C_1,R_{mod}^1)$
\end{algorithm}


\subsection{Perturbation and Ranking}
Combining DSL ranking tweaking and adding perturbed examples overcomes shortcomings of both techniques and reduces user input.\\ \\
\begin{algorithm}[H]
\caption{Generate robust program: Perturbation and Ranking}
    Given: original benchmark constraints $C_1$, DSL Ranker $R$ \\
    Generate new constraints $C_2$ using entity and character replacement in $C_1$, $C_2 = PERTURB(C_1)$\\
    $C= C_1\cup C_2$\\
    Create new ranker $R_{mod}^2$ by fixing delimiters such that each program in benchmarks sees same set of delimiters\\
    Synthesize robust program $P = SYNTHESIS(C,R_{mod}^2)$ 
\end{algorithm}

\subsection{Notes}
Please find below the revised algo for noisy landmark identification w.r.t to landmark inference.
Previously: 
•	In landmark hierarchy 
o	NoisyScore = (1/number of noisy landmarks + 1)
o	Noisy landmarks is defined the landmark regions containing landmark string which present outside of any ROI computed using output labels. 
o	NoisyScore is used as stopping condition for deciding whether to do more rounds of landmark inference.
•	ROI which is given as input to synthesis is always w.r.t base landmark, outer and middle landmarks in hierarchy are used as anchors to reach to the correct base landmark using nearest landmark logic.

Current:
•	In landmark hierarchy
o	Noisy landmarks definition is changed slightly only for base landmark.
	Noisy landmarks for base landmark is defined as the landmark regions satisfying one more condition apart from this. Any base landmark string S which also occurs outside of the ROIs (R1, R2,…Rn) when grown from noisy base LB’ to a region R’ (using steps computed using LB, R1), if R’ structure is same as any of structures in (R1, R2,…Rn) then base landmark S is noisy.
	Since we have ROI structure filtering at inference time, region grown from incorrect base landmarks will be filtered out.
o	If R’ structure is same as we have in Getthere Name field, one more round of hierarchy is done. If R’ is different as we have in Qatar then we stop at base landmark only and therefore have only Departure as landmark now, no mobile number is learnt as hierarchy. 
o	With this change we now do not need to compute all base landmarks at inference, we revert to the original logic of picking up nearest landmark in hierarchy. 
	We did multiple base landmarks for Qatar because there was 1 mobile number but 2 Departure but now we have only Departure as landmark. 
o	Rest of landmarks in hierarchy obey the previous definition of noisy landmarks since these are not concerned with ROI. 

Important note:
•	With this reverting back to nearest landmark logic at inference, code is assuming that hierarchy is only of this pattern (L1 -> L2 -> L3 -> ..)* which says each ROI is associated with unique L1, L2, ..

\end{comment}


==> robustness.tex <==

In the previous paragraph, we did not constrain the extractors produced in
any way.
%
However, in practice, we want the produced extractors to \emph{generalize} to
unseen input documents.
%
Intuitively, given a new input document $\doc$ that is ``similar'' to the
example inputs, the extractor should produce the output regions that
``correspond'' to the example output regions.
%
The notions of ``similar'' and ``correspond'' cannot be defined
globally---not only do they depend on the application domain, but also the
specific application that is under consideration.

In this section, we provide a brief overview of the various desirable characteristics of an extraction algorithm. Though this list is not exhaustive in any sense, it provides us a compass to reason about extraction quality and robustness.

\begin{itemize}
    \item Extraction should be agnostic to changes in regions outside of ~$\regionofinterest$ regions
    \item Extraction should be agnostic to changes in the $\regionofinterest$ regions
    \item Extraction should be agnostic to permutations of the various regions
    \item Extraction should be agnostic to the number of occurrences of the various regions
\end{itemize}

\begin{example}
  Let's consider Figure~\ref{fig:htmlextraction}~again. The goal of the extraction here is to extract various fields related to flight bookings. 
  \begin{itemize}
      \item An extraction program for flight departure time should be agnostic to the changes in the \textit{Car} block highlighted in the red. Ideally, this program should also be agnostic to any changes outside of the departure time blocks marked in green.
      \item An extraction program should be robust to changes within the green highlighted regions, for instance, \textit{Depart} is changed to \textit{Departure} or the structure of the green region is changed.
      \item The \textit{Air} and \textit{Flight} can be permuted in arbitrary ways, and the extraction program should be robust to such changes.
      \item Likewise, these blocks can occur multiple times and the extraction program should be agnostic to such changes.
  \end{itemize}
  \end{example}

We propose Hierarchical Synthesis algorithm $\resyn$ which incorporates the robustness characterizations described above. $\resyn$ synthesizes programs that are robust to outside region changes, permutations and occurrence of various regions, and is robust to within region changes to some extent.

\begin{comment}
We consider two types of extractors: models and programs.
%
For a given set of examples $\Examples$, models and programs are produced
using machine learning and program synthesis techniques, respectively.
%
These two classes of techniques have very different and complementary
characteristics.
%
Machine learning techniques often require a large number of training
examples, necessarily produce unsound extractors, and the produced models
generalize to unseen inputs extremely well.
%
On the other hand, program synthesis techniques require few training
examples, produce sound extractors, and are limited in generalizing to unseen
inputs.
\end{comment}

%
 \begin{comment}
% \begin{example}
  In the scenario from Section~\ref{sec:motivation}, where the task is to
  extract departure times from flight reservation emails, an extractor learnt
  from the example can be reasonably expected to generalize to emails in the
  same format.
  %
  Further, a user typically expects the extractor to also generalize to
  variants of the format: for example, in emails of a similar format, but
  with advertisement blocks between paragraphs.
  %
  However, as we move further away from the original format, the less likely
  it is that an extractor will be able to correctly extract departure times.
  %
  Hence, to measure robustness, it is necessary to define a set of admissible
  inputs, i.e., the domain of inputs on which the extractor is expected to
  work.
  
% \begin{comment}
  An additional difficulty in specifying robustness is that the desired
  extractor depends on the \emph{user's intention} in addition to the
  provided examples $\Examples$.
  %
  In Section~\ref{sec:motivation}, we implicitly assumed that the intention
  behind the example is ``extract all flight departure times''.
  %
  However, there are multiple possible intents: for example, ``extract both
  departure and arrival times for both forward and return flights'',
  ``extract departure times for the forward flights'', ``extract departure
  times for the forward flights of only the first passenger'', etc.
  %
  Hence, it is impossible to define a notion of robustness based purely on
  the inputs provided to the extraction system.
\end{comment}
  %
% \end{example}
% \end{comment}

\begin{comment}
As shown in the example above, we follow a very pragmatic approach towards
measuring robustness: using \emph{admissible inputs} and a \emph{golden
extractor}.
%
The set of admissible inputs $\adocs \subseteq \docs$ is a set of documents
similar to the example inputs.
%
The golden extractor $\Extractor^* : \adocs \to \Regions$ is an extractor
that operates only on $\adocs$ and captures the user's intent on those
documents.
%
We say that an extractor is \emph{robust} if $\forall \doc \in \adocs. \;
\Extractor(\doc) = \Extractor^*(\doc)$.
%
Note that $\adocs$ and $\Extractor^*$ are not provided as inputs to the
extraction task, but concepts that help us measure define and measure
robustness in our experiments.
\end{comment}
%

